A Framework for Combining Entity Resolution and Query Answering in Knowledge Bases

We propose a new framework for combining entity resolution and query answering in knowledge bases (KBs) with tuple-generating dependencies (tgds) and equality-generating dependencies (egds) as rules. We define the semantics of the KB in terms of special instances that involve equivalence classes of entities and sets of values. Intuitively, the former collect all entities denoting the same real-world object, while the latter collect all alternative values for an attribute. This approach allows us to both resolve entities and bypass possible inconsistencies in the data. We then design a chase procedure that is tailored to this new framework and has the feature that it never fails; moreover, when the chase procedure terminates, it produces a universal solution, which in turn can be used to obtain the certain answers to conjunctive queries. We finally discuss challenges arising when the chase does not terminate.

==> 00-Abstract/abstract.tex <==
\begin{abstract}
	In this paper....
\end{abstract}

==> 04-KER/KER.tex <==

\renewcommand{\Mod}{\mathit{Sol}}

\newcommand{\Emp}{\mathit{Emp}}
\newcommand{\Pers}{\mathit{Pers}}
\newcommand{\CI}{\mathit{CI}}
\newcommand{\phone}{\mathit{phone}}
\newcommand{\name}{\mathit{name}}
\newcommand{\comp}{\mathit{comp}}
% \newcommand{\Yahoo}{\textbf{Yahoo}}
% \newcommand{\IBM}{\textbf{IBM}}
\newcommand{\Yahoo}{\textnormal{\textbf{Yahoo}}}
\newcommand{\IBM}{\textnormal{\textbf{IBM}}}
\newcommand{\director}{\mathit{dir}}
\newcommand{\CEO}{\mathit{CEO}}


\section{Framework}
\label{sec:framework}

In this section we define the KBs that we study in this paper. We remark that whereas we adopt standard notions at the syntax level, the semantics we propose is novel, since it accounts for merging entities and values, as informally discussed in the introduction.

\subsection{Syntax}

A \emph{knowledge base (KB)} $\K$ is a pair $(\T,\DB)$, where $\T$ is a \emph{TBox} %, which models intensional knowledge, 
and $\DB$ is a \emph{database}. 
%(also called ABox in the Description Logics and ontologies parlance).
%\nb{this might be changed if the ABox and TBox are already defined in the introduction} 
%%
The TBox is a finite set of \emph{tuple-generating dependencies} (tgds) and \emph{equality-generating dependencies} (egds).  
%
A \emph{tgd} is a formula of the form:
%% 
\begin{align}
	\label{eq:tgd}
	\begin{array}{c}
		\forall \vec{x}(\phi(\vec{x}) \rightarrow \exists \vec{y} \psi(\vec{x}, \vec{y}))
	\end{array}
\end{align}
%%
where $\phi(\vec{x})$ and $\psi(\vec{x},\vec{y})$  are built-in free and constant free conjunctions of atoms of the form~(\ref{eq:conj}), such that $\vec{x} \cap \vec{y} = \emptyset$. As in \cite{FKMP05}, we assume that all the variables in $\vec{x}$ appear in $\phi(\vec{x})$ but not necessarily in $\psi(\vec{x}, \vec{y}))$. We call $\phi(\vec{x})$ the body of the tgd, and $\psi(\vec{x},\vec{y})$ the head of the tgd.%\nb{unclear whether we can extend to generic conjunctions of atoms (i.e., allow constants). However, it is better to stay simple - it is already a very general form of dependency} 

%\begin{example}
%	\label{ex:TBox}
%	Let $\T$ be the TBox containing the following tgds:	    			
%	\begin{align*}
%		\arraycolsep=3.0pt
%		\begin{array}{ll}
%			t_1) & Professor(x)  \rightarrow Person(x)    					\\
%			t_2) & Person(x)  \rightarrow \exists y.has\_name(x,y)			\\
%			t_3) & teaches(x,y)   \rightarrow Professor(x) \\
%			t_4) & lives\_in(x,y)  \rightarrow City(y)
%		\end{array}
%	\end{align*}
%	Such a TBox states that professors are persons ($t_1$), every person has a name ($t_2$), who teaches something is a professor ($t_3$), who lives somewhere lives in a City ($t_4$). \qed
%\end{example}

%%

An \emph{egd} is a formula of the form:
\begin{equation}
	\label{eq:egd}
	\forall \vec{x}(\phi(\vec{x}) \ra  y = z)
\end{equation}
where $\phi(\vec{x})$ is a conjunction of atoms of the form~(\ref{eq:conj}) and $y$ and $z$ are distinct variables in $\vec{x}$, such that both $y$ and $z$ are either entity-variables (in this case we call the formula \emph{entity-egd}) or value-variables (in this case we call the formula \emph{value-egd}). We call $\phi(\vec{x})$ the body of the egd.


%We then distinguish between:
%\begin{itemize}
%	\item \emph{entity-egds}, which are rules of the form~(\ref{eq:egd}) where both the variables $y$ and $z$ are entity-variables. 
%	\item \emph{value-egds}, which are rules of the form~(\ref{eq:egd}) where both the variables $y$ and $z$ are value-variables;
%\end{itemize}

In the following, we may write tdgs and egds without the universal and existential quantification over the variables. 
%(i.e., we may omit $\forall \vec{x}$ and the associated parentheses).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PREVIOUS EXAMPLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{example}
%	\label{ex:TBox}
%	Let $\T$ be the TBox containing the following rules:	    			
%	\begin{align*}
%		\arraycolsep=3.0pt
%		\begin{array}{ll}
%			t_1) & Professor(x)  \rightarrow Person(x)    					\\
%			t_2) & Person(x)  \rightarrow \exists y.has\_name(x,y)			\\
%			t_3) & teaches(x,y)   \rightarrow Professor(x) \\
%			t_4) & lives\_in(x,y)  \rightarrow City(y) \\
%			t_5) & has\_name(x,y) \wedge has\_name(x,z) \rightarrow %\rightleftharpoons(y, z) \\
%			y=z\\
%			t_6) & Person(x) \wedge Person(y) \wedge lives\_in(x,z) \wedge lives\_in(y,z) \\
%		& \wedge has\_name(x,t) \wedge has\_name(y,w) \wedge jaccardsim(t, w, 0.7) \rightarrow %{\sim}(x, y)
%		x=y
%		\end{array}
%	\end{align*}
%	Such a TBox states that professors are persons ($t_1$), every person has a name ($t_2$), who teaches something is a professor ($t_3$), who lives somewhere lives in a City ($t_4$). Every individual has only one name ($t_5$). Finally the last egd ($t_6$) states that if two entities denoting persons live in the same place and the Jaccard similarity of their names is higher than $0.9$, they are denoting the same real-world person. \qed
%	%related to each other by the $\sim$ relation. \qed
%\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{example}
	\label{ex:TBox}
	Let $\T$ be the TBox containing the following rules:
	\begin{align*}
        \small
		\arraycolsep=0.0pt
		\begin{array}{ll}
			r_1) & \Emp(p,\comp) \rightarrow \Pers(p)    					\\
			r_2) & \CI(p, \name_1, \phone_1) \wedge \CI(p, \name_2, \phone_2)\\ 
                 &   \rightarrow \name_1 = \name_2 \\
            r_3) & \CI(p,\name_1,\phone_1)\wedge \CI(p,\name_2,\phone_2)\\ 
                 &  \rightarrow \phone_1=\phone_2 \\
            r_4) & \CI(p_1,\name,\phone)\wedge \CI(p_2,\name,\phone) \rightarrow p_1=p_2 \\
			r_5) & \Pers(p_1) \wedge \Pers(p_2) \wedge \Emp(p_1,\comp) \wedge \Emp(p_2,\comp) \wedge\\ 
                 &  \CI(p_1,\name_1,\phone_1) \wedge \CI(p_2,\name_2,\phone_2) \wedge\\
		       &   \JaccardSim(\name_1,\name_2,0.6) \rightarrow p_1 = p_2
		\end{array}
        \normalsize
	\end{align*}
% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{ll}
% 			t_1) & Emp(id,comp) \rightarrow Pers(id)    					\\
% 			t_2) & CI(id, name_1, address_1) \wedge CI(id, name_2, address_2) \rightarrow name_1 = name_2 \\
% 			t_3) & CI(id_1,name,address)\wedge CI(id_1,name,address) \rightarrow id_1=id_2 \\
% 			t_4) & Pers(id_1) \wedge Person(id_2) \wedge Emp(id_1,comp) \wedge Emp(id_2,comp) \wedge CI(id_1,name_1,address_1) \\
% 		& \wedge CI(id_2,name_2,address_2) \wedge JaccardSim(name_1,name_2,0.9) \rightarrow id_1 = id_2
% 		\end{array}
% 	\end{align*}
	
		We have that $\type(\Emp) = \tup{\entity,\entity}$, $\type(\Pers) = \tup{\entity}$, and $\type(\CI) = \tup{\entity,\val,\val}$. 
		The predicate $\Pers$ denotes a set of persons, $\Emp$ associates employees to the companies they work for, and $\CI$ maintains contact information of entities, i.e., name and home landline phone number.
		%Finally $JaccardSim$ is a ternary built-in predicate which checks that the Jaccard similarity between two strings (first two arguments) is above a certain threshold (third argument).\nb{see comment in the introduction about JaccardSim} 
		The rules in the TBox state that every employee is a person ($r_1$), an entity can have only one name ($r_2$), an entity can have only one landline phone ($r_3$), and two entities with the same name and landline phone are indeed denoting the same individual ($r_4$). 
  The last formula ($r_5$) states that if two persons work in same company and the Jaccard similarity of their names is higher then $0.6$ then they are indeed the same person.
%	
%	Here we have that the relation $Emp$ reports employees and their respective companies, also $type(Emp) = \tup{\entity,\entity}$, the unary relation $Pers$ stores the persons and $type(Pers) = \tup{\entity}$ and finally $CI$ contains the contact informations such as name and address and $type(CI) = \tup{\entity,\val,\val}$. Finally $Jaccard$ is an 3-ary built-in predicate representing the jaccard similarity between two strings. \nb{FIX}
%	Such a TBox states that every employee is a person ($t_1$), an individual can have only one name ($t_2$) and two individual with the same address and name are the same entity. The last formula states that if two persons are employees in same company and the jaccard similary of their names is higher then $0.9$ then they are denoting the same-real world entity. \nb{FIX the similarity value and text!!!!}
\qed	
\end{example}


%Note that by imposing certain restrictions to the value-egds, it is possible to express functionalities over attributes typical of some DLs.
%
%
 %\begin{example}
%	\label{ex:TBox}
%	Let $\T$ be the TBox containing the following assertions:	    			
%	\begin{align*}
%		\arraycolsep=3.0pt
%		\begin{array}{ll}
%			t_1) & Professor(x)  \rightarrow Person(x)    					\\
%			t_2) & Person(x)  \rightarrow \exists y.has\_name(x,y)			\\
%			t_3) & teaches(x,y)   \rightarrow Professor(x) \\
%			t_4) & lives\_in(x,y)  \rightarrow City(y) \\
%			t_5) & has\_name(x,y) \wedge has\_name(x,z) \rightarrow y=z
%					& Person(x) \wedge Person(y) \wedge lives\_in(x,z) \wedge lives\_in(y,z)\\
%		& \wedge has\_name(x,t) \wedge has\_name(y,w) \wedge jaccardsim(t, w, 0.9) \rightarrow {\sim}(x, y)
%		\end{aligned}
%		\end{array}
%	\end{align*}
%	Such a TBox states that professors are persons ($t_1$), every person has a name ($t_2$), who teaches something is a professor ($t_3$), who lives somewhere lives in a City ($t_4$). Finally every individual has only one name ($t_5$) \qed
%\end{example}
%
%


%%\subsection{Assertional component}

%The ABox $\A$ %in a $\KER$ system  
%is formed by a finite set of membership assertions on atomic concepts, atomic roles, and attributes. Such assertions have the form:
%%%
%\begin{align*}
%	\arraycolsep=20.0pt
%	\begin{array}{llll}
%		C(e) & R(e_1,e_2)  & A(e,v)
%	\end{array}
%\end{align*}
%%%
%where $e,e_1,e_2 \in \mathsf{N_E}$ and $v \in \mathsf{N_V}$. Intuitively, $C(e)$ states that the entity $e$ is an instance of the atomic concept $C$. $R(e_1,e_2)$ states that the pair constituted by the entities $e_1$ and $e_2$ is an instance of the atomic role $R$. $A(e,v)$ states that the pair constituted by the entity $e$ and the value $v$ is an instance of the  attribute $A$.



 

The database $\DB$ of a KB $\K$ is a finite set of ground atoms over the alphabets $\alphaPredicates$, $\alphaEntities$, and $\alphaValues$, that is, formulas of the form $P(c_1,\ldots,c_n)$ where $P \in \alphaPredicates$, and each $c_i$ is either an entity from  $\alphaEntities$, if $\type(P,i)=\entity$, or a value from $\alphaValues$, if $\type(P,i)=\val$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PREVIOUS EXAMPLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{example}
%	\label{ex:DB}
%	Let $\DB$ be the database containing the following assertions:
%	\begin{align*}
%		\arraycolsep=3.0pt
%		\begin{array}{llcll}
%			a_1) & Professor(\textbf{\#Ullman}) & & a_9) & lives\_in(\textbf{\#Ullman}, \textbf{\#Palo.Alto}) \\
%			a_2) & Professor(\textbf{\#A.Einstein}) & & a_{10}) & lives\_in(\textbf{\#J.Ullman}, \textbf{\#Palo.Alto}) \\
%			a_3) & Professor(\textbf{\#Einstein}) & & a_{11}) & has\_name(\textbf{\#Ullman}, \texttt{Ullman}) \\
%			a_4) & Person(\textbf{\#J.Ullman}) & & a_{12}) & has\_name(\textbf{\#J.Ullman}, \texttt{J.Ullman}) \\
%			a_5) & Person(\textbf{\#Einstein.A}) & & a_{13}) & has\_name(\textbf{\#A.Einstein}, \texttt{A.Einstein}) \\		
%			a_6) & teaches(	\textbf{\#Ullman}, \textbf{\#Database}) & & a_{14}) & has\_name(\textbf{\#Einstein}, \texttt{Einstein}) \\
%			a_7) & lives\_in(\textbf{\#Einstein}, \textbf{\#Zurich}) & & a_{15}) & has\_name(\textbf{\#Einstein.A}, \texttt{Einstein.A}) \\
%			a_8) & lives\_in(\textbf{\#A.Einstein}, \textbf{\#Zurich}) \\
%		\end{array}
%	\end{align*}
%	This database states that \textbf{\#Ullman}, \textbf{\#A.Einstein}, \textbf{\#Einstein} are professors (assertions $a_1$, $a_2$, and $a_3$), \textbf{\#J.Ullman} and \textbf{\#Einstein.A} are persons ($a_4$, $a_5$), \textbf{\#Ullman} teaches \textbf{\#Database} ($a_6$), both \textbf{\#Einstein} and \textbf{\#A.Einstein} live in \textbf{\#Zurich} ($a_7$, $a_8$), and both \textbf{\#Ullman} and \textbf{\#J.Ullman} live in \textbf{\#Palo.Alto} ($a_9$, $a_{10}$).
%	
%	Finally the name of \textbf{\#Ullman} is \texttt{Ullman}, the name of \textbf{\#J.Ullman} is \texttt{J.Ullman} ($a_{11}$, $a_{12}$), the name of \textbf{\#A.Einstein} is \texttt{A.Einstein} ($a_{13}$), the name of \textbf{\#Einstein} is \texttt{Einstein} ($a_{14}$), and the name of \textbf{\#Einstein} is \texttt{Einstein.A} ($a_{15}$). 
%	\qed
%\end{example}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}
	\label{ex:DB}
	Let $\DB$ be the database containing the following ground atoms:
	\begin{align*}
        \small
		\arraycolsep=5.0pt
  %       \begin{array}{llll}
		% 	d1) & Emp(\textbf{\#Doe$_1$}, \textbf{\#Yahoo}) & d4) & CI(\textbf{\#Doe$_1$}, \texttt{J. Doe}, \texttt{34-435}) \\
		% 	d2) & Emp(\textbf{\#Doe$_2$}, \textbf{\#Yahoo}) & d5) & CI(\textbf{\#Doe$_2$}, \texttt{John Doe}, \texttt{35-263}) \\
		% 	d3) & Emp(\textbf{\#Doe$_3$}, \textbf{\#IBM}) & d6) & CI(\textbf{\#Doe$_3$}, \texttt{Mary Doe}, \texttt{34-435}) \\
  %           & & d7) & CI(\textbf{\#Doe$_4$}, \texttt{J. Doe}, \texttt{35-263}) \\
		% \end{array}
        \begin{array}{llll}
			g_1) & \Emp(\Doe_1, \Yahoo) & g_4) & \CI(\Doe_1, \texttt{J. Doe}, \PNumberA) \\
			g_2) & \Emp(\Doe_2, \Yahoo) & g_5) & \CI(\Doe_2, \texttt{John Doe}, \PNumberB) \\
			g_3) & \Emp(\Doe_3, \IBM) & g_6) & \CI(\Doe_3, \texttt{Mary Doe}, \PNumberA) \\
            & & g_7) & \CI(\Doe_4, \texttt{J. Doe}, \PNumberB) \\
		\end{array}
	\end{align*}
% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{ll}
% 			d1) & Emp(\textbf{\#J.Doe}, \textbf{\#Yahoo}) \\
% 			d2) & Emp(\textbf{\#John Doe}, \textbf{\#Yahoo}) \\
% 			d3) & Emp(\textbf{\#Mary Doe}, \textbf{\#IBM}) \\
% 			d4) & CI(\textbf{\#J.Doe}, \texttt{J.Doe}, \texttt{avenue 25}) \\
% 			d5) & CI(\textbf{\#John Doe}, \texttt{John Doe}, \texttt{avenue 28}) \\
% 			d6) & CI(\textbf{\#Mary Doe}, \texttt{Mary Doe}, \texttt{avenue 25}) \\
% 			d7) & CI(\textbf{\#JD}, \texttt{J. Doe}, \texttt{avenue 28}) \\
% 		\end{array}
% 	\end{align*}
	$\DB$ specifies that $\Doe_1$ and $\Doe_2$ are employees of $\Yahoo$ ($g_1$,$g_2$), $\Doe_3$ is an employee of $\IBM$ ($g_3$), $\Doe_1$ has name \texttt{J.Doe} and phone number \PNumberA\ ($g_4$), $\Doe_2$ has name \texttt{John Doe} and phone number \PNumberB\ ($g_5$), $\Doe_3$ has name \texttt{Mary Doe} and phone number \PNumberA\ ($g_6$), and finally $\Doe_4$ has name \texttt{J. Doe} and phone number \PNumberB\ ($g_7$).
	\qed
\end{example}

To ensure that built-in predicates have the same semantics in every KB, 
%are pre-interpreted and thus ground atoms over such symbols are always the same in all KBs, 
we assume to have a fixed (infinite and countable) set $GB$ of ground atoms of the form  $B(v_1,..v_n)$, where $B \in \alphaBuiltIns$ and $v_1,..v_n$ belong to $\alphaValues$. Intuitively, $GB$ contains all facts over built-in predicates that hold overall. 
%
Then, given a KB $\K=(\T,\DB)$, we assume that $\DB=\DB_O \cup \DB_B$, where $\DB_O$ contains only ground atoms with predicate from $\alphaOntology$ and $\DB_B$ is the set of all atoms in $GB$ whose built-in predicates and values are mentioned in $\T$ and $\DB_O$.

% More heavy version (BTW, it has an error)
%let $GB_\K$ be the set of all ground atoms constructible from built-in predicates occurring in the rules of $\T$ and values from $\alphaValues$ occurring in $\K$ (i.e., in the database $\DB$ or in the rules of $\T$), we assume that $\DB=\A \cup  \S$, where $\A$ is a finite set of ground atoms whose predicates belong to $\alphaOntology$ and  $\S= GB_\K \cap GB$. Note that also $\S= GB_\K \cap GB$ is finite, since $GB_\K$ is finite.
%%
%%Note: built-Ins are not allowed in queries. We might allow in query, but the query has to be safe, i.e., if a variable occur in an atom whose predicate is a built-in, it must occur in a non-builtin atom in the query. This ensures that such variable can be assgined only to set of values occurring in the database, or containing nulls, but in particular avoids that we ask queries such us `b'=`b', which is evidently true, but is not evaluated as such over the database if `b' is not mentioned in the database.

\subsection{Semantics}
\label{sec:KERsemantics}


We first introduce two additional infinite, countable and disjoint sets $\alphaEntityNulls$ and $\alphaValueNulls$ that are also disjoint from all the alphabets mentioned in Section~\ref{sec:predicates-atoms-conjunctions}. %and are such that $\alphaEntityNulls\cap\alphaValueNulls=\emptyset$. 
We call $\alphaEntityNulls$ and $\alphaValueNulls$ the set of entity-nulls and the set of value-nulls, respectively, whereas their union is simply referred to as the set of nulls.
%%
Moreover, we use 
%
%$\powerset(\Sigma)$ to denote the power set of a set $\Sigma$, $\powersetnoempty(\Sigma)$ to denote $\powerset(\Sigma) \setminus \emptyset$, and 
$\sig(\K)$ to denote the signature of a KB $\K$, i.e., the set of symbols from $\alphaPredicates$, $\alphaEntities$ and $\alphaValues$ occurring in $\K$. 

%The semantics of a KB is given in terms of tailored structures\nb{not sure ``structure'' is the right term} that associate predicate arguments ranging over entities to classes of entities and entity-nulls computed with respect to a given equivalence relation, and associate predicate arguments ranging over values to non-empty sets of values and value-nulls. This is formalized through the notion of instance of a KB.

%Intuitively, 
The semantics of a KB is given in terms of special databases, called KB instances, containing ground atoms that, instead of constants, have as components either equivalence classes of entities and entity-nulls or non-empty sets of values and value-nulls, depending on the type of the corresponding predicate argument. This idea is formalized below.

\begin{definition}(instance of a KB)
\label{def:instance}
Given a KB $\K$, a set $\mathcal{S} \subseteq (\alphaEntities \cap \sig(\K)) \cup \alphaEntityNulls$, and an equivalence relation $\sim$ over $\mathcal{S}$. An \emph{instance $\I$ for $\K$ \wrt $\sim$} is a set of facts\nb{maybe (but I am not sure) we need a different term, to distinguish them from standard facts, which we however call ground atoms in the paper. I was not able to find an appropriate term (set-based facts?).} of the form $P(\genericSet_1,\ldots,\genericSet_n)$ such that $P \in \alphaPredicates \cap \sig(\K)$, $\arity(P)=n$, and, for each $1 \leq i \leq n$, $T_i \neq \emptyset$ and either $T_i \in \mathcal{S}/\sim$, if $\type(P,i)=\entity$, or $T_i \subseteq (\alphaValues \cap \sig(\K)) \cup \alphaValueNulls$, if $\type(P,i)=\val$. The relation $\sim$ is also called the equivalence relation associated to $\I$.
\end{definition}

To denote an equivalence class occurring in $\I$, we may use the symbol $E$ (possibly with subscript) or $[e]_\sim$ (or simply $[e]$, when $\sim$ is clear from the context), where $e$ is any element of the equivalence class. We remark that an equivalence class $E$ occurring in $\I$ may contain both entities and entity-nulls. In the following we however may simply refer to $E$ as an equivalence class of entities\nb{Maybe this is misleading, but saying every time that the set contains also nulls is very heavy}. Analogously, a non-empty subset of $(\alphaValues \cap \sig(\K)) \cup \alphaValueNulls$ occurring in $\I$ can be simply referred to as a set of values, denoted with the symbol $V$ (possibly with subscript). We will instead use $\genericSet$ (possibly with subscript) to denote a set that can be either an equivalence class of entities or a set of values. 

%
% old version: interpretations
%
%\begin{definition}[interpretation]
%	\label{def:interpretation}
%%%
%Given a KB $\K$, an \emph{interpretation $\I$ of $\K$} is a triple $(\Delta^\I,\sim^\I,\cdot^\I)$, such that:
%\begin{itemize} 
%	\setlength\itemsep{0.2em}
%\item $\Delta^\I= \Delta^\I_E \cup\Delta^\I_V$, where $\Delta^\I_E$ and $\Delta^\I_V$ are two disjoint sets such that  $\Delta^\I_E=(\alphaEntities \cap \sig(\K)) \cup \Delta^\I_{E_\bot}$ and $\Delta^\I_V=(\alphaValues \cap \sig(\K)) \cup \Delta^\I_{V_\bot}$, where $\Delta^\I_{E_\bot} \subseteq \alphaEntityNulls$ and $\Delta^\I_{V_\bot} \subseteq \alphaValueNulls$;
%
%\item ${\sim}^\I $ is an equivalence relation over $\Delta^\I_E$;
%\item $\cdot^\I$ is an interpretation function that maps:
%%%
%\begin{itemize}
%	\setlength\itemsep{0.2em}
%	\item each entity $e \in \alphaEntities \cap \sig(\K)$ to a set $\Int{e}=[e]_{\sim^\I}$;
%	\item each value $v \in \alphaValues \cap \sig(\K)$ to itself;
%	\item each $n$-ary predicate $P \in \alphaPredicates \cap \sig(\K)$ to a set $\Int{P} \subseteq \prod_{i=1}^n \Gamma_i$, where either $\Gamma_i=\Delta^\I_E/{\sim^\I}$ if $\type(P,i)=\entity$ or $\Gamma_i=\powersetnoempty({\Delta^\I_V})$ if $\type(P,i)=\val$, for $1\leq i \leq n$; %\footnote{We recall that $\Delta^\I_E/{\sim^\I}$ is the quotient set of  $\sim^\I$ on $\Delta^\I_E$}
%\end{itemize}
%\end{itemize}
%
%\end{definition}
%
%According to the above definition, we have that: each entity occurring in $\K$ is interpreted by the equivalence class the entity belongs to; each value occurring in $\K$ is interpreted by itself (in all interpretations); an $n$-ary predicate $P$ occurring in $\K$ is interpreted by a set of $n$-tuples, such that each of their components is either an equivalence class from $\Delta^\I_E/{\sim^\I}$ %, i.e., the quotient set of  $\sim^\I$ on $\Delta^\I_E$, 
%or a non-empty set of elements from $\Delta_V^\I$, depending on whether the type of the corresponding argument in $P$ is $\entity$ or $\val$, respectively.
%%; an $n$-ary predicate $B \in \alphaPredicates$ is interpreted by a set of $n$-tuples whose components are non-empty subsets of $\alphaValues$. 
%%%
%%We assume that the semantics of built-in predicates is the same in all interpretations, that is, given a KB $\K$ and  any two interpretations $\I_i$ and $\I_j$, of $\K$, $B^{\I_i}=B^{\I_j}$ for each $B \in \alphaBuiltIns$. Thus, from now on, we will omit to say how an interpretation interprets built-in predicates.
%%%
%%In the same spirit, we can avoid to always specify how values in $\alphaValues$ are interpreted. 
%%  
%
%Given a $n$-ary predicate $P$, %$P \in \alphaPredicates \cup \alphaBuiltIns$, 
%if a tuple $\tup{T_1,\ldots,T_n}$ belongs to $P^\I$ we say that $P^\I(\genericSet_1,\ldots,\genericSet_n)$ is a \emph{$P$-fact of $\I$}. The set of all $P$-facts of $\I$ is denoted by $\Facts(P,\I)$. Moreover, $\Facts(\I)= \bigcup_{P \in \alphaPredicates} \Facts(P,\I)$. An element of $\Facts(\I)$ is simply called a fact of $\I$, when we do not need to refer to its predicate (facts of an interpretation have not to be confused with facts of databases, being the latter ground atoms, as defined in Section~\ref{sec:preliminaries}).
%
%To simplify notation, when $\I$ is clear from the context, we may also denote a $P$-fact of $\I$ as $P(T_1,\ldots,T_n)$. Similarly, for an equivalence class $[e]_{\sim^\I}$ we may omit to indicate the equivalence relation $\sim^\I$, and simply write $[e]$. Moreover, from now on, when we refer to an equivalence class $E$ of entities (resp.\ set $\V$ of values) occurring in an interpretation, we mean the $E$ (resp.\ $V$) may contain both entities and entity-nulls (resp.\ values and value-nulls).

The active domain of an instance $\I$ for $\K$ is the set containing all equivalence classes and all sets of values occurring in $\I$, as formalized below, where we also give the notion of underlying domain.

\begin{definition}[active and underlying domain]
	Given a KB $\K$ and an instance $\I$ for $\K$ \wrt an equivalence relation $\sim$. The \emph{active domain of $\I$} is the set
	$
	\activeD(\I) = \{\genericSet \mid \textrm{there exist } P(\genericSet_1,\ldots,\genericSet_n) \in \I \textrm{ and } i \in \{1,\ldots, n\}\textrm{ such that } T=T_i\}$. 	
	With $\activeD_E(\I)$ and $\activeD_V(\I)$, we denote the set of all sets of entities and the set of all sets of values contained in $\activeD(\I)$, respectively. Obviously $\activeD(\I)=\activeD_E(\I) \cup \activeD_V(\I)$.
	
		Then, the \emph{underlying domain of $\I$} is the set $\underD(\I)=\underD_E(\I) \cup \underD_V(\I)$, where $\underD_E(\I)= \{e~|~\textrm{there exists }\entitySet \in \activeD_E(\I)\textrm{ and } e \in \entitySet\}$ and $\underD_V(\I)= \{v~|~\textrm{there exists }\valueSet \in \activeD_V(\I)\textrm{ and } v \in \valueSet\}$.
\end{definition}

It is not difficult to see that if $\I$ is an instance of $\K$ \wrt an equivalence relation $\sim$ over a set $\S \subseteq (\alphaEntities \cap \sig(\K)) \cup \alphaEntityNulls$, then $\I$ is an instance of $\K$ \wrt the equivalence relation $\sim'$ over $\underD_E(\I)$ such that $\sim'=\sim \setminus \{\tup{n_i,n_j}~|~n_i,n_j  \not \in \underD_E(\I)\}$. Moreover $\S/\sim \supseteq \underD_E(\I) /\sim'$ and $\sim'$ is unique, i.e., there is no $\sim'' \neq \sim$ such that $\sim''$ is an equivalence relation over $\underD_E(\I)$ and $\I$ is an instance for $\K$ \wrt $\sim''$. Therefore, in the following we will consider only instances \wrt equivalence relations over $\S=\underD_E(\I)$.
%%\nb{In principle $\mathcal{S}$, by definition, might contain also entity-nulls that do not appear in $\underD_E(\I)$, but if we ``project'' the equivalence relation $\sim$ to the set $\underD_E(\I)$, we obtain an equivalence relation with the same equivalence classes of entities.}.
Furthermore, we may simply call $\I$ an instance for $\K$ and leave the equivalence relation associated to $\I$ implicit. %The relation $\sim$ is also called the equivalence relation associated to $\I$.
%%Moreover, an instance $\I$ for $\K$ w.r.t.\ $\sim$ (over a set $\mathcal{S}$) can be simply referred to as an instance for $\K$, when $\sim$ (and $\mathcal{S}$) can be understood from the context.\nb{In this way, later on, we can simply talk about a solution for a KB} 



%% Comment: Note that it also holds that every equivalence class appears in $\active_E(\I)$. Indeed, every element $e$ involved in $\sim$ occur in a set of $\active_E(\I)$, which implies that such set is in fact the equivalence class $[e]_\sim$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PREVIOUS EXAMPLE (uses interpretations) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{example}
%	\label{ex:interpretation}
%Let $\Delta^I$ be a set containing exactly the entities and the values mentioned in Example~\ref{ex:DB}, $\sim^\I$ be an equivalence relation only specifying that each entity is equivalent to itself, and $\cdot^\I$ be an interpretation  function mapping each entity $e$ to the singleton set containing $e$, and the predicate $Person$, $Professor$, $teaches$, $lives\_in$, and $has\_name$ as follows:
%%%
%\[
%\begin{array}{lcl}
%Person^\I&=&\{[\textbf{\#J.Ullman}],[\textbf{\#Einstein.A}],[\textbf{\#Ullman}],[\textbf{\#Einstein}],[\textbf{\#A.Einstein}]\}\\
%Professor^\I&=&\{[\textbf{\#Ullman}],[\textbf{\#A.Einstein}],[\textbf{\#Einstein}]\}\\
%City^\I&=&\{[\textbf{\#Zurich}]\}\\
%teaches^\I&=&\{\tup{[\textbf{\#Ullman}],[\textbf{\#Database}]}\}\\
%leaves\_in^I&=&\{\tup{[\textbf{\#Einstein}],[\textbf{\#Zurich}]},\tup{[\textbf{\#A.Einstein}],[\textbf{\#Zurich}]},\tup{[\textbf{\#Ullman}],[\textbf{\#Palo.Alto}]},\\
%&&\tup{[\textbf{\#J.Ullman}],[\textbf{\#Palo.Alto}]}\}\\
%has\_name^\I&=&\{\tup{[\textbf{\#Ullman}],\{\texttt{Ullman}\}},\tup{[\textbf{\#J.Ullman}],\{\texttt{J.Ullman}\}},\tup{[\textbf{\#A.Einstein}],\{\texttt{A.Einstein}\}},\\
%&&\tup{[\textbf{\#Einstein}],\{\texttt{Einstein}\}},\tup{[\textbf{\#Einstein.A}],\{\texttt{Einstein.A}\}}\}
%\end{array}
%\]
%%%
%Then, $\I=(\Delta^\I,\sim^\I,\cdot^\I)$ is an interpretation.
%%%
%Consider now $\Delta^{\I'}=\Delta^\I$, $\sim^{\I'}$ such that
%%%
%\[
%\begin{array}{lcl}
%\Delta^{\I'}/\sim^{\I'} &=&\{[\textbf{\#J.Ullman},\textbf{\#Ullman}],[\textbf{\#Einstein},\textbf{\#A.Einstein}],[\textbf{\#Einstein.A}],[\textbf{\#Database}],\\
%&&[\textbf{\#Zurich}],[\textbf{\#Palo.Alto}]\}
%\end{array}
%\]
%%%
%and $\cdot^{\I'}$ defined as follows
%%%
%\[
%\begin{array}{lclcl}
%\textbf{\#J.Ullman}^{\I'}&=&\textbf{\#Ullman}^{\I'}&=&[\textbf{\#J.Ullman},\textbf{\#Ullman}]\\
%\textbf{\#Einstein}^{\I'}&=&\textbf{\#A.Einstein}^{\I'}&=&[\textbf{\#Einsteinn},\textbf{\#A.Einstein}]\\
%\textbf{\#Einstein.A}^{\I'}&=&[\textbf{\#Einstein.A}]\\
%\textbf{\#Database}^{\I'}&=&[\textbf{\#Database}]\\
%\textbf{\#Palo.Alto}^{\I'}&=&[\textbf{\#Palo.Alto}]\\
%\end{array}	
%\]
%%%
%\[
%\begin{array}{lcl}
%	Person^{\I'}&=&\{[\textbf{\#J.Ullman},\textbf{\#Ullman}],[\textbf{\textbf{\#Einstein},\#A.Einstein}],[\textbf{\#Einstein.A}]\}\\
%	Professor^{\I'}&=&\{[\textbf{\#J.Ullman},\textbf{\#Ullman}][\textbf{\textbf{\#Einstein},\#A.Einstein}]\}\\
%	City^{\I'}&=&\{[\textbf{\#Zurich}]\}\\
%	teaches^{\I'}&=&\{\tup{[\textbf{\#J.Ullman},\textbf{\#Ullman}],[\textbf{\#Database}]}\}\\
%	leaves\_in^{\I'}&=&\{\tup{[\textbf{\textbf{\#Einstein},\#A.Einstein}],[\textbf{\#Zurich}]},\tup{[\textbf{\#J.Ullman},\textbf{\#Ullman}],[\textbf{\#Palo.Alto}]}\}\\
%	has\_name^{\I'}&=&\{\tup{[\textbf{\#J.Ullman},\textbf{\#Ullman}],\{\texttt{Ullman}\}},\tup{[\textbf{\#Einstein.A}],\{\texttt{Einstein.A}\}},\\
%	&&\tup{[\textbf{\textbf{\#Einstein},\#A.Einstein}],\{\texttt{Einstein},\texttt{A.Einstein}\}}\}
%\end{array}
%\]
%%%
%Then, also $\I'=(\Delta^{\I'},\sim^{\I'},\cdot^{\I'})$ is an interpretation. \qed
%	\end{example}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}
	\label{ex:interpretation}
Let $\K=(\T,\DB)$ be a KB such that $\T$ and $\DB$ are as in Example~\ref{ex:TBox} and in Example~\ref{ex:DB}, respectively. 
%
%
% version for interpretations
%
%Then, consider $\I=(\Delta^\I,\sim^\I,\cdot^\I)$, such that $\Delta^\I=\Delta^\I_E \cup \Delta^\I_V$, with $\Delta^\I_E$ and $\Delta^\I_V$ be the sets of entities and values occurring in $\K$, respectively, $\sim^\I$ i the identity on $\Delta^\I_E$, and $\cdot^\I$ is such that $\Facts(\I)$ contains the following facts:
%
Then, consider %$\sim^\I$ 
%$\sim$  to be the identity on $\underD_E(\I)$, and 
the following set $\I$ of facts:
%%
\small
\[
\begin{array}{l}
\Pers([\Doe_1]),~~\Pers([\Doe_2]),~~\Pers([\Doe_3])\\ 
\Emp([\Doe_1], [\Yahoo]),~~\Emp([\Doe_2], [\Yahoo]),\\
\Emp([\Doe_3], [\IBM]),\\
\CI([\Doe_1], \{ \texttt{J. Doe} \}, \{ \PNumberA \} ),\\ 
\CI([\Doe_2], \{ \texttt{John Doe} \}, \{ \PNumberB \} ),\\
CI([\Doe_3], \{ \texttt{Mary Doe} \}, \{ \PNumberA \}),\\ 
CI([\Doe_4], \{ \texttt{J. Doe} \}, \{ \PNumberB \}).
\end{array}
\]
\normalsize
%%
It is easy to see that $\I$ is an instance for $\K$ \wrt the identity relation over the set $\mathcal{S}=\{\Doe_1,\Doe_2,\Doe_3,\Doe_4,\Yahoo,\IBM\}$.
%
% old: uses intepretations
%
%It is easy to see that $\I$ obeys the condition of Definition~\ref{def:interpretation}, and thus it is an an interpretation.
%
%As a further example of interpretation, consider $\I'$ such that $\Delta^{\I'}=\Delta^{\I}$ and $\Facts(\I')$ consists of the following facts ($\sim^{\I'}$ can be understood accordingly):
%

As a further example, consider the equivalence relation $\sim'$ over the set $\mathcal{S}$, such that $\Doe_1 \sim' \Doe_2 \sim' \Doe_4$ are the only equivalences in $\sim'$ different from the identity. The following set of facts $\I'$ is an instance for $\K$ \wrt $\sim'$.
%
\[
\small
\begin{array}{l}
\Pers([\Doe_1,\Doe_2,\Doe_4]),~\Pers([\Doe_3]),\\
\Emp([\Doe_1,\Doe_2,\Doe_4],[\Yahoo]),~\Emp([\Doe_3],[\IBM]),\\
\CI([\Doe_3],\{ \texttt{Mary Doe} \},\{ \PNumberA \}),\\
\CI([\Doe_1,\Doe_2,\Doe_4], \{\texttt{J. Doe},\texttt{John Doe} \}, \{\PNumberA,\PNumberB\} ).
%\multicolumn{2}{l}{\CI([\Doe_1,\Doe_2,\Doe_4], \{ \texttt{J. Doe}, \texttt{John Doe} \}, \{ \PNumberA, \PNumberB \} ).}
\normalsize
\end{array}
\]
\qed
\end{example}



%
%old (uses interpretations)
%
%Given an interpretation $\I$ for a KB $\K$, 
%the active domain of $\I$ is the set of equivalence classes in $\Delta_E^\I/{\sim^\I}$ and subsets of $\Delta_V^\I$ that occur in $\Int{P}$, for some predicate $P$, %$P \in \alphaPredicates \cap sig(\K)$,
%%%
%as formalized below, where we also give the notion of underlying domain.
%
%\begin{definition}[active and underlying domain]
%	Given an interpretation $\I$ for a KB $\K$, the \emph{active domain of $\I$} is the set
%	$
%	\activeD(\I) = \{\genericSet \mid \textrm{there exists } P(\genericSet_1,\ldots,\genericSet,\ldots,\genericSet_n) \in \Facts(\I)\}
%    $
%	
%	With $\activeD_E(\I)$, we denote the set of all equivalence classes contained in $\activeD(\I)$, whereas with $\activeD_V(\I)$ we denote the set of all subsets of $\Delta_V^\I$ contained in $\activeD(\I)$. Obviously $\activeD(\I)=\activeD_E(\I) \cup \activeD_V(\I)$
%	
%	
%	Then, the \emph{underlying domain of $\I$} is the set $\underD(\I)=\underD_E(\I) \cup \underD_V(\I)$, where $\underD_E(\I)= \{e~|~\textrm{there exists }\entitySet \in \activeD_E(\I)\textrm{ and } e \in \entitySet\}$ and $\underD_V(\I)= \{v~|~\textrm{there is }\valueSet \in \activeD_V(\I)\textrm{ and } v \in \valueSet\}$.
%\end{definition}
%
%In words, whereas the active domain contains the sets (of entities of values) 
%used to interpret predicates, the underlying domain is the set of all elements occurring in an equivalence class in $\activeD_E(\I)$ or in a set of $\activeD_V(\I)$. 


To define the notions of satisfaction of tgds and egds by an instance, we first introduce the notion of assignment from a conjunction $\phi(\vec{x})$ of atoms to an instance $\I$ of a KB $\K$. To formalize this definition, we need to describe a preliminary transformation of $\phi(\vec{x})$ that substitutes each occurrence of a value-variable in $\phi(\vec{x})$ with a fresh variable. We call such fresh variables \emph{set-variables}. More precisely, with $\trasf(\phi(\vec{x}))$ we denote a conjunction of atoms obtained as follows
%%
\begin{tabbing}
	for each\= ~value-variable $x$ in $\vec{x}$\\
	\> for each\= ~occurrence of $x$ in $\phi(\vec{x})$:\\
	\>\> replace $x$ with a fresh symbol $S$ 
\end{tabbing}

Given a value-variable $x$ in $\vec{x}$, we write $\setvar(x,\trasf(\phi(\vec{x})))$ to denote the set of fresh variables used in $\trasf(\phi(\vec{x}))$ to replace the occurrences of $x$ in $\phi(\vec{x})$.
%%
For instance, if $\phi(\vec{x}) =P_1(x,y,z),P_2(y,z),P_3(x,w)$, where $\type(P_1)=\tup{\entity,\entity,\val}$, $\type(P_2)=\tup{\entity,\val}$, and $\type(P_3)=\tup{\entity,\val}$, then $\trasf(\phi(\vec{x}))=P_1(x,y,S_1^z),P_2(y,S_2^z),P_3(x,S_1^w)$, where  $S_1^z$, $S_2^z$, $S_1^w$ are the fresh set-variables introduced by $\trasf$. Also, $\setvar(z,\trasf(\phi(\vec{x})))=\{S_1^z,S_2^z\}$ and  $\setvar(w,\trasf(\phi(\vec{x})))=\{S_1^w\}$. 
As just done, hereinafter, for each value-variable $x$, each set-variable in $\setvar(x,\trasf(\phi(\vec{x})))$ will have $x$ as superscript.

%
We are now ready to formally define assignments. 
%%In the definition, without loss of generality, we assume that every atom in $\trasf(\phi(\vec{x}))$ has the form $P(x_1,\ldots,x_j,S_1,\ldots S_k, e_1, \ldots, e_\ell, v_1, \ldots, v_m)$, where $x_1,\ldots,x_j$ are entity-variables, $S_1,\ldots S_k$ are set-variables, $e_1,\ldots,e_\ell$ are entities in $\alphaEntities$, $v_1,\ldots,v_m$ are values in $\alphaValues$, $j,k,\ell,m$ are all greater than or equal to $0$ and $j+k+\ell+m \geq 1$.

\begin{definition}[assignment]
	\label{def:assignment-revisited}
	Let $\phi(\vec{x})$ be a conjunction of atoms of the form~(\ref{eq:conj}),
	and let $\I$ be an instance for a KB $\K$ \wrt to an equivalence relation $\sim$ over $\underD_E(\I)$. An \emph{assignment from $\phi(\vec{x})$ to $\I$} is a mapping $\mu$ from the variables and values in $\tau(\phi(\vec{x}))$ to $\activeD(\I)$, defined as follows:
	\begin{enumerate}	
		\item $\mu(x)$ is an equivalence class in $\activeD_E(\I)$, for every entity-variable $x$; %in $\vec{x}$;
		\item  $\mu(v)=\valueSet$ such that 
	$\valueSet \in \activeD_V(\I)$ and $v \in \valueSet$, for every value $v$; % in $\phi(\vec{x})$;		
		\item  $\mu(S)$ is a set of values in $\activeD_V(\I)$, for every set-variable $S$; % in $\trasf(\phi(\vec{x}))$;
		\item $\bigcap_{i=1}^{k} \mu(S_i^x) \neq \emptyset$, for every value-variable $x$ such that $\setvar(x,\trasf(\phi(\vec{x})))=\{S_1^x,\ldots,S_k^x\}$; 
	%
	% old: uses interpretations
	%
%		\item $\Facts(\I)$ contains a $P$-fact of the form $P^\I(\mu(x_1),\ldots,\mu(x_j),\mu(S_1),\ldots \mu(S_k), e_1^\I, \ldots, e_\ell^\I, \mu(v_1), \ldots, \mu(v_m))$, for each atom $P(x_1,\ldots,x_j,S_1,\ldots S_k, e_1, \ldots, e_\ell, v_1, \ldots, v_m)$ of $\trasf(\phi(\vec{x}))$.
% 
% old: uses a more general form of atom (but in the end not completely general)
%
%		\item $\I$ contains a fact of the form $P(\mu(x_1),\ldots,\mu(x_j),\mu(S_1),\ldots \mu(S_k), [e_1]_\sim, \ldots, [e_\ell]_\sim, \mu(v_1), \ldots, \mu(v_m))$, for each atom $P(x_1,\ldots,x_j,S_1,\ldots S_k, e_1, \ldots, e_\ell, v_1, \ldots, v_m)$ of $\trasf(\phi(\vec{x}))$.
		\item $\I$ contains a fact of the form $P(\mu(x),\mu(S),[e]_\sim,\mu(v))$, for each atom $P(x,S,e,v)$ of $\trasf(\phi(\vec{x}))$, where $x$ is entity-variable, $S$ is a set-variable, %replacing an occurrence of a value-variable in $\phi(\vec{x})$, 
    $e$ is an entity in $\alphaEntities$ and $v$ is a value in $\alphaValues$ (the definition can be generalized in the obvious way for atoms of different form).\nb{This has been simplified wrt the previous version. We indeed used atoms of the form $P(x_1,\ldots,x_j,S_1,\ldots S_k, e_1, \ldots, e_\ell, v_1, \ldots, v_m)$, but it seems to be enough to consider $P(x,S,e,v)$ }
	\end{enumerate}	
	%%
 \end{definition} 


In words, the above definition says that an assignment maps every entity-variable to an equivalence class of entities (Point~1), every value to a set of values containing it (Point~2),  and every occurrence of a value-variable to a set of values (Point~3), in such a way that multiple occurrences of the same value-variable are mapped to sets with a non-empty intersection (Point~4). This condition captures the intuition that, since predicate arguments ranging over values are interpreted through sets of values, a join between such arguments holds when such sets have a non-empty intersection. Finally, Point~5 states that the conjunction $\phi(\vec{x})$ has an instantiation in $\I$.\nb{is `instantiation' clear? check also `instantiated' in the sentence below}
We remark that the assignment above defined also maps values to sets of values (Point~2). This indeed allows the assignment to map atoms in the conjunction $\phi(\vec{x})$ to facts in $\I$, since predicate arguments ranging over values are instantiated in $\I$ with sets of values.


Given an atom $P(\vec{t})$ of $\phi(\vec{x})$, % (see equation~(\ref{eq:conj})), 
with $\mu(P(\vec{t}))$ we denote the fact of $\I$ described at Point~5 of Definition~\ref{def:assignment-revisited}, and call it the \emph{$\mu$-image (in $\I$) of $P(\vec{t})$}. Moreover, with $\mu(\phi(\vec{x}))$ we denote the set $\{ \mu(P(\vec{t}))~|~P(\vec{t})\textrm{ occurs in } \phi(\vec{x})\}$ and call it the \emph{$\mu$-image (in $\I$) of $\phi(\vec{x})$}.

%% OLD - no longer needed  
%In the following, it will be also convenient to refer to the \emph{$\mu$-image (in $\I$) of a predicate $P$}, denoted $\mu(P)$, defined as the image of the conjunction of atoms obtained by eliminating from $\phi(\vec{x})$ all atoms whose predicate is different from $P$. Note that if $\phi(\vec{x})$ contains only one atom with predicate $P$, this last notion coincides with the $\mu$-image of such atom.


\begin{example}
	\label{ex:assignment}
%%
%% we can decomment if we want to reuse another example of assignement (a bit trivial)
%% 
%	Consider the instance $\I'$ in Example~\ref{ex:interpretation} and the egd $r_3$ in Example~\ref{ex:TBox}. Apply $\tau$ to the body of $r_3$ and get: 
%\[
%\CI(p_1,S_1^{\name},S_1^{\phone})\wedge \CI(p_2,S_2^{\name},S_2^{\phone}) 
%\]
%Let $\mu$ be a mapping defined as follows:
%\[
%\small
%\begin{array}{lclcl}
%	\hat{\mu}(p_1)&=&\hat{\mu}(p_2)&=&[\textbf{\#Doe$_1$}\textbf{\#Doe$_2$}\textbf{\#Doe$_4$}]\\
%	\hat{\mu}(S_1^{name})&=&\hat{\mu}(S_2^{name})&=& \{ \texttt{J. Doe}, \texttt{John Doe} \}\\
%	\hat{\mu}(S_1^{phone})&=&\hat{\mu}(S_2^{phone})&=&\{ \PNumberA, \PNumberB \}
%\end{array}
%\normalsize
%\]
%Then, $\hat{\mu}$ is an assignment from the body of $t_3$ to $\I'$.

%
% old stuff: it could be deleted
%
% 	Consider now the ternary predicate $PersInfo$, such that $\type(PersInfo)=\tup{\entity,\val,\val}$, and the ternary predicate $SameAge$, such that  $\type(SameAge)=\tup{\entity,\entity,\val}$. In words, $PersInfo$ is a used to store personal data, and in particular to associate an entity denoting a person (first argument) with her/his age and height (second and third argument, respectively), whereas $SameAge$ is putting together pairs of people having the same age.
% 	%%
% 	Let $\T$ be a TBox containing only the tgd $PersInfo(x_1,y,z) \land PersInfo(x_2,y,w)  \ra SameAge(x_1,x_2,y)$. Intuitively, the TBox is saying that two persons with the same age have to occur also as instances of the predicate $SameAge(x_1,x_2,y)$ (together with the age). Let now $\I''$ be an interpretation such that the following holds:
% 	\[
% 	\begin{array}{l}
% 	\mathbf{\#e_1}^{\I''}=[\mathbf{\#e_1}]\\
% 	\mathbf{\#e_2}^{\I''}=[\mathbf{\#e_2}]\\
% 	PersInfo^{\I''}=\{\tup{[\mathbf{\#e_1}],\{12,13\},\{160\}},\tup{[\mathbf{\#e_2}]},\{13,14\},\{155\}\}\\
% 	SameAge^{\I''}=\{\tup{[\mathbf{\#e_1}],[\mathbf{\#e_2}],\{13\}}\}
% 	\end{array}
% 	\]
% 	Let us now apply the transformation $\tau$ to the body of the previous tgd, and obtain $PersInfo(x_1,S_1^y,S^z) \land PersInfo(x_2,S_2^y,S^w)$ , and let $\mu$ be a mapping to the active domain of $\I$ defined as follows 
% 	\[
% \begin{array}{lcl}
% 	\mu(x_1)&=&[\mathbf{\#e_1}]\\
% 	\mu(x_2)&=&[\mathbf{\#e_2}]\\
% 	\mu(S_1^y)&=&\{12,13\}\\
% 	\mu(S_2^y)&=&\{13,14\}\\
% 	\mu(S^z)&=&\{160\}\\
% 	\mu(S^w)&=&\{155\}
% \end{array}
% \]
% It is easy to see that $\mu$ is an assignment from the body of the tdg to $\I$. Similarly, let us apply $\trasf$ to the head of the tdg and obtain 	$SameAge(x_1,x_2,S^y)$, and let us define $\mu'$ as follows 
% 	\[
% \begin{array}{lcl}
% 	\mu'(x_1)&=&[\mathbf{\#e_1}]\\
% 	\mu'(x_2)&=&[\mathbf{\#e_2}]\\
% 	\mu'(S^y)&=&\{13\}
% \end{array}
% \]
% Then, $\mu'$ is an assignment from the head of the tgd to $\mu'$.
%
Let $\SameHouse$ be a ternary predicate such that $\type(\SameHouse)=\tup{\entity,\entity,\val}$, %, which put together pairs of people living in the same house, as well as their home phone number.
	%%
and let $r_0$ be the tgd $\CI(p_1,\name_1,\phone) \wedge \CI(p_2,\name_2,\phone)  \ra \SameHouse(p_1,p_2,\phone)$.
% \small
% $$\CI(p_1,\name_1,\phone) \wedge \CI(p_2,\name_2,\phone)  \ra \SameHouse(p_1,p_2,\phone)$$ 
% \normalsize
 In words, $r_0$ states that two entities with the same landline phone number also live in the same house. %(phone number is also repeated in $\SameHouse$ facts). 
 Then, let $\T$ be the TBox in Example~\ref{ex:TBox}, $\T' = \T \cup \{ r_0 \}$, and $\K'=(\T',\DB)$, where $\DB$ is as in Example~\ref{ex:DB}. Finally, let $\I''$ be
	the instance of $\K'$ obtained by adding to $\I'$ of Example~\ref{ex:interpretation} the fact $\SameHouse([\Doe_1,\Doe_2,\Doe_4],[\Doe_3],\{ \PNumberA, \PNumberC \})$.
%
% old: uses interpretations
%	
%	Let now $\I''$ be an interpretation such that the following holds:
%	
%	\[
%	\begin{array}{l}
%	\mathbf{\textbf{\#Doe$_1$}}^{\I''}=[\textbf{\#Doe$_1$}]\\
%	\mathbf{\textbf{\#Doe$_3$}}^{\I''}=[\textbf{\#Doe$_3$}]\\
%	CI^{\I''}([\mathbf{\textbf{\#Doe$_1$}}],\{\texttt{J.Doe}\},\{\PNumberA,\PNumberB\})\\
%	CI^{\I''}([\mathbf{\textbf{\#Doe$_3$}}],\{\texttt{Mary Doe}\},\{\texttt{211-4959}, \PNumberA\})\\
%	SameHouse^{\I''}([\mathbf{\textbf{\#Doe$_1$}}],[\mathbf{\textbf{\#Doe$_3$}}],\{ \PNumberA \})
%	\end{array}
%	\]
%
% \[
% \begin{array}{l}
% 	CI([\mathbf{\textbf{\#Doe$_1$}}],\{\texttt{J. Doe}\},\{\PNumberA,\PNumberB\})\\
% 	CI([\mathbf{\textbf{\#Doe$_3$}}],\{\texttt{Mary Doe}\},\{\texttt{211-4959}, \PNumberA\})\\
% 	SameHouse([\mathbf{\textbf{\#Doe$_1$}}],[\mathbf{\textbf{\#Doe$_3$}}],\{ \PNumberA \})
% \end{array}
% \]
% \[
% \begin{array}{l}
% 	SameHouse([\mathbf{\textbf{\#Doe$_1$}\textbf{\#Doe$_2$}\textbf{\#Doe$_4$}}],[\mathbf{\textbf{\#Doe$_3$}}],\{ \PNumberA \})
% \end{array}
% \]
	Let us now apply %the transformation 
 $\tau$ to the body of $r_0$ and obtain $\CI(p_1,S^{\name_1},S_1^{\phone}) \land CI(p_2,S^{\name_2},S_2^{\phone})$, and let $\mu$ be %a mapping to the active domain of $\I''$ 
 defined as follows: 
	\[
\begin{array}{lcl}
	\mu(p_1)&=&[\Doe_1,\Doe_2,\Doe_4]\\
	\mu(p_2)&=&[\Doe_3]\\
	\mu(S^{\name_1})&=&\{\texttt{J. Doe},\texttt{John Doe}\}\\
	\mu(S^{\name_2})&=&\{\texttt{Mary Doe}\}\\
	\mu(S_1^{\phone})&=&\{\PNumberA,\PNumberB\}\\
	\mu(S_2^{\phone})&=&\{\PNumberA\}.
\end{array}
\]
It is easy to see that $\mu$ is an assignment from the body of %the tdg 
 $r_0$ to $\I''$ (note the non-empty intersection between  $\mu(S_1^{\phone})$ and $\mu(S_2^{\phone})$). Let us now apply $\trasf$ to the head of $r_0$, which returns $\SameHouse(p_1,p_2,R^{\phone})$. The following mapping $\mu'$ is an assignment from $\SameHouse(p_1,p_2,\phone)$
to $\I''$:
	\[
\begin{array}{lcl}
	\mu'(p_1)&=&[\Doe_1,\Doe_2,\Doe_4]\\
	\mu'(p_2)&=&[\Doe_3]\\
	\mu'(R^{\phone})&=&\{\PNumberA,\PNumberC\}
\end{array}
\]
%Then, $\mu'$ is an assignment from $\SameHouse(p_1,p_2,\phone)$
%to $\I''$.
\qed
\end{example}

We are now ready to define the semantics of tgds and egds. 
%%

\begin{definition}[rule satisfaction]
\label{def:rule-satisfaction}
An instance $\I$ for a KB $\K$ satisfies:
%%
\begin{itemize}
\item a tgd of the form (\ref{eq:tgd}), if for each assignment $\mu$ from	$\phi(\vec{x})$ to $\I$ there is an assignment $\mu'$ from  $\psi(\vec{x}, \vec{y})$ to $\I$ such that 
\begin{itemize}
	\item $\mu(x)=\mu'(x)$, for each entity-variable $x$ in $\vec{x}$;
	\item $\bigcap_{i=1}^{k} \mu(S_i^x) \subseteq \bigcap_{i=1}^{\ell} \mu'(R_i^x)$, for each value-variable $x$ in $\vec{x}$, where $\{S_1^x,\ldots,S_k^x\}=\setvar(x,\trasf(\phi(\vec{x})))$ and $\{R_1^x,\ldots,R_\ell^x\}=\setvar(x,\trasf(\psi(\vec{x},\vec{y})))$;
	\end{itemize}
We call each such $\mu'$ a %\emph{$\psi(\vec{x},\vec{y})$compatible tgd-extension}
\emph{head-compatible tgd-extension} of $\mu$ to $\I$ (or simply a tgd-extension of $\mu$ to $\I$). 
% if $\psi(\vec{x},\vec{y})$ is clear from the context)
\item an entity-egd of the form (\ref{eq:egd}), if each assignment $\mu$ from $\phi(\vec{x})$ to $\I$ is such that $\mu(y)=\mu(z)$;
\item a value-egd of the form (\ref{eq:egd}), if each assignment $\mu$ from $\phi(\vec{x})$ to $\I$ is such that
$\mu(S^y)=\mu(S^z)$ for each set-variable $S^y,S^z \in \setvar(y,\trasf(\phi(\vec{x}))) \cup \setvar(z,\trasf(\phi(\vec{x})))$.
\end{itemize} 
\end{definition}
%%Let us comment about the previous notions of rule satisfaction. 
%%Obviously, $\I$ satisfies a rule if there is no assignment from the rule body to $\I$.
%%
In words, given a rule $r$, for each assignment $\mu$ from the body of $r$ to $\I$, the above definition is formalizing what follows: $(1)$ if $r$ is a tgd, the definition specifies two different behaviours on frontier variables, i.e., variables occurring in both the body and the head of the tgd, depending on whether they are entity-variables or value-variables. Namely, for the tgd to be satisfied, it has to be possible to extend $\mu$ so that $(i)$ every frontier entity-variable is assigned with exactly the same equivalence class both in the body and the head of the rule (which is in line with the standard semantics for frontier variables in tgds), and $(ii)$ the intersection of the sets of values assigned in the body of the tgd to the various occurrences of a frontier value-variable $x$ is contained in the intersection of the sets of values assigned to the occurrences of $x$ in the head of the tgd. Indeed, whereas $\mu$ maps all the occurrences of an entity-variable in $\phi(\vec{x})$ to the same  equivalence class, it may map multiple occurrences of a value-variable to different sets of values with non empty-intersection. Thus it is somehow natural that the tgd propagates such intersection.
%%
$(2)$ If $r$ is an entity-egd, the notion of satisfaction is somehow standard, since it requires that $\mu$ assigns $y$ and $z$ to the same equivalence class of entities. $(3)$ If $r$ is a value-egd, to somehow replicate the same behaviour we have for entity-egds, we have again to take into account that each occurrence of $y$ in the rule body can be assigned by $\mu$ to a different set of values (provided that all such sets have a non-empty intersection), and analogously for each occurrence of $z$. The definition thus simply asks that all such sets are equal, for the value-egd to be satisfied.
%This definition captures the idea that an egd should be read as a matching dependency, and, as we will see more in detail in the next section, in the case the egd is not satisfied by an instance $\I$, it is always possible to modify $\I$ by replacing all sets assigned to the occurrences of $y$ and $z$


\begin{example}
%%
%% we can decomment if we want to reuse the other example of assignement from Ex 4
%%
%%Instance $\I'$ from Example~\ref{ex:assignment} satisfies the entity-egd $r_3$ of Example ~\ref{ex:TBox}. Indeed, the assignment $\hat{\mu}$ shown in Example~\ref{ex:assignment} is the only assignment from the body of $r_3$ to $\I'$ and $\hat{\mu}$ is such that $\mu(p_1)=\mu(p_2)$. 
%%
%Moreover, 
$\I''$ from Example~\ref{ex:assignment} satisfies the tgd $\CI(p_1,\name_1,\phone) \land \CI(p_2,\name_2,\phone)  \ra \SameHouse(p_1,p_2,phone)$, since $\mu'$ is a head-compatible tgd extension of the only assignment $\mu$ from the body of the tgd to $\I''$. Indeed, $\mu'(p_1)=\mu(p_1)$, $\mu'(p_2)=\mu(p_2)$, and $\mu'(S^{\phone})=\mu(S_1^{\phone}) \cap \mu(S_2^{\phone})$ (cf.\ Example~\ref{ex:assignment}).
%since for the only assignment $\mu$ from the body of the tgd to $\I''$, shown in Example~\ref{ex:assignment}, %there is $\mu'$ such that $\mu'(p_1)=\mu(p_1)$, $\mu'(p_2)=\mu(p_2)$, and $\mu'(S^{phone})=\mu(S_1^{phone}) \cap \mu(S_2^{phone})$ (cf.\ Example~\ref{ex:assignment}). 
It is then also easy to see that instance $\I'$ from Example~\ref{ex:assignment} satisfies all rules of Example ~\ref{ex:TBox}.
\qed
\end{example}

We can then say that a TBox $\T$ of a KB $\K$ is satisfied by an instance $\I$ for $\K$ if $\I$ satisfies all tgds and egds in $\T$.

To complete the semantics of a KB $\K=(\T,\DB)$, we have to state when an instance $\I$ for $\K$ satisfies $\DB$.
%%
Given a ground atom $P(c_1,\ldots,c_n)$ in $\DB$, 
%where $P$ is an $n$-ary predicate from $\alphaPredicates$ and $c_1,\ldots,c_n$ are constants such that each $c_i$ is either an entity or a value, depending on the type of the $i$-th argument of $P$, and an interpretation $\I$, 
we say that $\I$ satisfies $P(c_1,\ldots,c_n)$ if there exists a fact  $P(\genericSet_1,\ldots,\genericSet_n)$ in $\I$ such that $c_i \in \genericSet_i$, for $1\leq i \leq n$. We also note that, if $\type(P,i)=\entity$, then %$\genericSet_i=[c_i]_{\sim^{\I}}$.
$\genericSet_i=[c_i]$. 
Obviously, $\I$ satisfies a database $\DB$ if $\I$ satisfies all ground atoms in $\DB$. 
%%%
Finally, we say that $\I$ is a \emph{solution} for a  KB $\K=\tup{\T,\DB}$, denoted as $\I \models \K$, if $\I$ satisfies $\T$ and $\DB$. The set of all solutions of a KB $\K$ is denoted with $\Mod(\K)$, i.e., $\Mod(\K) = \{ \I~|~\I \models \K \}$.

\begin{example}
	It is not difficult to see that instance $\I$ given in Example~\ref{ex:interpretation} does not satisfy the KB described in Example~\ref{ex:TBox} and Example~\ref{ex:DB}, whereas instance $\I'$ in Example~\ref{ex:interpretation} is a solution for such KB. \qed
\end{example}

We conclude this part by introducing some notations that will be useful for the following treatment.

\begin{definition}  \label{def:contain} 	Let $\vec{\genericSet}=\tup{\genericSet_1,\ldots,\genericSet_n}$ and
	$\vec{\genericSet'}=\tup{\genericSet'_1,\ldots,\genericSet'_n}$ be two tuples in which each $\genericSet_i$ and each $\genericSet'_i$ is either a set of entities and entity-nulls or a set of values and value-nulls. We say that: 
		
	
	\begin{itemize} 
		\item $\vec{\genericSet}$ and $\vec{\genericSet'}$ are \emph{equal}, denoted $\vec{\genericSet}=\vec{\genericSet'}$, if $\genericSet_i = \genericSet'_i$ for every $1 \leq i \leq n$.
		\item $\vec{\genericSet'}$ \emph{dominates} $\vec{\genericSet}$ (or analogously $\vec{\genericSet}$ is dominated by $\vec{\genericSet'}$), denoted $\vec{\genericSet} \leq \vec{\genericSet'}$, if $\genericSet_i \subseteq \genericSet'_i$,  for every $1 \leq i \leq n$. If  $\vec{\genericSet} \leq \vec{\genericSet'}$ and $\vec{\genericSet} \neq \vec{\genericSet'}$, we say that $\vec{\genericSet'}$ \emph{strictly dominates} $\vec{\genericSet}$, and denote it $\vec{\genericSet} < \vec{\genericSet}'$. 
		
		\item given two facts $P(\vec{\genericSet})$ and $P(\vec{\genericSet'})$, $P(\vec{\genericSet'})$ \emph{dominates} $P(\vec{\genericSet})$ (or analogously $P(\vec{\genericSet})$  is dominated by $P(\vec{\genericSet'})$), denoted $P(\vec{\genericSet}) \leq P(\vec{\genericSet'})$, if $\vec{\genericSet} \leq \vec{\genericSet'}$, and  $P(\vec{\genericSet'})$ \emph{strictly dominates} $P(\vec{\genericSet})$, denoted $P(\vec{\genericSet}) < P(\vec{\genericSet'})$, if $\vec{\genericSet} < \vec{\genericSet'}$.
	\end{itemize}
	
\end{definition}



\subsection{Universal solutions}
\label{sec:univ-model}
Among all possible solutions of a KB, we characterize those having some special properties, called universal solutions, which are well understood and effectively used in standard approaches to theories of tgds and egds (see, e.g., \cite{FKMP05,CaGK13,CDLLR07}). The definition of universal solution males use of homomorphism between instances. Below, we provide a notion of homomorphism tailored to our framework.


\begin{definition}[homomorphism]
	\label{def:homomorphism}
	Let $\I_1$ and $\I_2$  be two instances of a KB $\K$.
	An homomorphism $h:\I_1 \rightarrow \I_2$ is a mapping from the elements of $\underD(\I_1)$ to elements of $\underD(\I_2)$ such that:
	\begin{enumerate}
		\item $h(e)=e$, for every entity $e \in \underD_E(\I_1) \cap \alphaEntities$;
		\item $h(e_\bot) \in \underD_E(\I_2)$, for every entity-null $e_\bot \in  \underD_E(\I_1) \cap \alphaEntityNulls$;
		\item $h(v)=v$, for every value $v \in \underD_V(\I_1) \cap \alphaValues$;
		\item $h(v_\bot) \in \underD_V(\I_2)$, for every value-null $v_\bot \in \underD_V(\I_1) \cap \alphaValueNulls$;
%		\item for each $P(\genericSet_1,\ldots,\genericSet_n) \in \I_1$ there exists $P(\genericSettwo_1,\ldots,\genericSettwo_n) \in \I_2$ such that $h(\genericSet_i) \subseteq \genericSettwo_i$, for $1 \leq i \leq n$, where $h(\genericSet_i)=\{h(x) \mid x \in \genericSet_i)\}$.\\
		\item for each $P(\genericSet_1,\ldots,\genericSet_n) \in \I_1$ there exists $P(\genericSettwo_1,\ldots,\genericSettwo_n) \in \I_2$ such that $P(h(\genericSet_1),\ldots,h(\genericSet_n))\leq P(\genericSettwo_1,\ldots,\genericSettwo_n)$, where $h(\genericSet_i)=\{h(x) \mid x \in \genericSet_i)\}$, for $1 \leq i \leq n$.
  %%\nb{Should we also define $h(\tup{T_1,\ldots,T_n})$?It might be useful, e.g., for Proposition \ref{pro:query-under-homo}}
	\end{enumerate}
\end{definition}

In the following, we may denote $P(h(\genericSet_1),\ldots,h(\genericSet_n))$ with $h(P(\genericSet_1,\ldots,\genericSet_n))$, and may use $h(\tup{\genericSet_1,\ldots,\genericSet_n})$ to indicate the tuple $\tup{h(\genericSet_1),\ldots,h(\genericSet_n)}$.

We say that an instance $\I_1$ is homomorphically equivalent to an instance $\I_2$ if there is an homomorphism $h:\I_1 \rightarrow \I_2$ and an homomorphism $h':\I_2 \rightarrow \I_1$. It is then easy to see that the composition of two homomorphisms yields an homomorphism.\nb{We might also say that composition of an homomorphim with an assignment does not yield an assignment, and add a Proposition saying ``if there is $h:\I_1 \rightarrow \I_2$ and assignment $\mu$ from $\phi(\vec{x})$ to $\I_1$, then there is an assignment $\mu'$ from $\phi(\vec{x})$ to $\I_2$ such that $\mu(t) \subseteq \mu'(t)$ for a variable or value $t$ in $\phi(\vec{x}$''. The proof can be extracted from the proof of Proposition \ref{pro:query-under-homo}.}
%, and that the composition of a homomorphism with an assignment yields a new assignment. 
%To formalize the composition of homomorphism with an assignment, let $\phi(\vec{x})$ be a conjunction of atoms of the form (\ref{eq:conj}), $\I_1$ and $\I_2$ be two interpretations,  $h:\I_1 \rightarrow \I_2$ be an homomorphism, and $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$. The \emph{composition of $h$ with $\mu$}, denoted $h \circ \mu$, is a mapping from the variables and values in $\tau(\phi(\vec{x}))$ to the set $\activeD(\I_2)$ such that $(h \circ \mu)(t)=h(\mu(t))$ for every entity-variable, set-variable, or value $t$ occurring in $\tau(\phi(\vec{x}))$. It is easy to see that $(h \circ \mu)$ is an assignment from  $\tau(\phi(\vec{x}))$ to $\activeD(\I_2)$ according to Definition~\ref{def:assignment-revisited}.


		

We are now ready to provide the definition of universal solution. 

\begin{definition}[universal solution]
	\label{def:universal}
	Let $\K$ be a KB, then a \emph{universal solution} for $\K$ is a solution $\U \in \Mod(\K)$ such that for every solution $\I \in \Mod(\K)$ there exists an homomorphism $h: \U \rightarrow \I$.
\end{definition}

The universal solution is unique up to homomorphic equivalence.




==> 05-Query_Answering/query.tex <==
%\newcommand{\cert}{\mathit{cert}}

\section{Query answering}
\label{sec:query-answering}
A conjunctive query (CQ) $q$ is an open %first-order logic 
formula of the form:
\begin{equation}
	\label{eq:CQ}
	\exists \vec{y}\,conj(\vec{x}, \vec{y})
\end{equation}
where $\vec{x}$ and $\vec{y}$ are the free %(or distinguished) 
the existential %(or non-distinguished) 
variables of $q$, respectively, and $conj(\vec{x}, \vec{y})$ is a built-in free conjunction of atoms of the form~(\ref{eq:conj}).
%\footnote{TO BE DOUBLED CHECKED: Our approach applies straightforwardly to CQs in which sets of values from $\mathsf{N_V}$ may occur in exactly the same positions where single values from $\mathsf{N_V}$ may occur (as, e.g., in the query $\exists x,y . \mathit{age}(x,\{78,80\})$, which asks to verify the existence of an individual that is both $78$ and $80$ years old, or in the query $\exists x . \mathit{age}(x,y) \land y\nonemptyint \{78,80\}$, asking for the existence of some one that is either $78$ or $80$, or both). This would require to slightly modify Definition~\ref{def:assignment-revisited}. For the sake of presentation we do not consider this case (notice also that CQs containing sets of values can always be rewritten into equivalent unions of CQs with values only).}
%%.
%each of the form $C(t)$ or $R(t, t')$ or $A(t, t'')$, where $C$ is an atomic concept, $R$ is an atomic role, $A$ is an attribute, $t$ and $t'$ are entity-variables occurring in either $\vec{x}$ or $\vec{y}$, or entities in $\mathsf{N_E}$, $t''$ is a value-variable occurring in either $\vec{x}$ or $\vec{y}$  or values in $\mathsf{N_V}$. As usual, each variable in $\vec{x}$ or $\vec{y}$ occur  either always in entity-positions or always in value-positions.
The number of variables in $\vec{x}$ is the \emph{arity} of the query. %A CQ with no free variables is called Boolean CQ.\nb{I do not think we need BCQ} 
In the following, a CQ with free variables $\vec{x}$ may be denoted with $q(\vec{x})$.

Given a KB $\K$, an instance $\I$ for $\K$, and a CQ $q(\vec{x})$, where $\vec{x}=x_1,\ldots,x_n$, %the set of \emph{answers to $q$ over $\I$}, 
the \emph{answer to $q$ over $\I$}, denoted by $q^\I$, is the set of tuples 
$\tup{\genericSet_1,\ldots,\genericSet_n}$ such that there is an assignment $\mu$ from $conj(\vec{x}, \vec{y})$ to $\I$ and for $1 \leq i \leq n$ it holds: % that:
\begin{itemize}
\item $\genericSet_i = \mu(x_i)$, if $x_i$ is an entity-variable;
\item $\genericSet_i=\bigcap_{j=1}^{k}\mu(S_j^{x_i})$, where $\{S_1^{x_i},\ldots,S_k^{x_i}\}=\setvar(x_i,\trasf(conj(\vec{x},\vec{y})))$, if $x_i$ is a value-variable.
\end{itemize}
With a little abuse of terminology, we also say that the above $\mu$ is an assignment from $q(\vec{x})$ to $\I$.

\begin{example}
\label{ex:query}
 %    Consider a KB $\K$ whose database is constituted by the facts $has\_name(\Doe_1,\texttt{J.Doe})$ and $has\_name(\Doe_2, \texttt{J.Doe})$, and whose TBox is constituted by the entity-egd $has\_name(x_1,y),has\_name(x_2,y) \ra x_1=x_2$.
	% It is easy to see that, in every solution for $\K$, $\Doe_1$ and  $\Doe_2$ must belong to the same equivalence class, and that the (unary) answer tuple $\tup{\{\Doe_1,\Doe_2\}}$ is a certain answer to the query $q(x) \la has\_name(x,y)$. The answer tuple $\tup{\{\Doe_1\}}$ instead is not a certain answer, even if it satisfies condition $(i)$  of Definition~\ref{def:certain-answer}, since it does not respect condition $(ii)$  (analogously for the answer tuple $\tup{\{\Doe_2\}}$)
Consider the TBox $\T''$ obtained by adding to $\T$ of Example~\ref{ex:TBox} the tgd $\Emp(p,\comp) \rightarrow \CEO(\comp,\director) \wedge \Pers(\director)$, which states that every company in which employees work has a CEO who is a person, and the entity-egd $\CEO(\comp,\director_1) \wedge \CEO(\comp,\director_2) \rightarrow \director_1 = \director_2$, which states that a company has exactly one CEO. Then, let
$\DB'$ be the database obtained by adding to $\DB$ of Example~\ref{ex:DB} the ground atom $CEO(\Yahoo,\Doe_1)$. Let now $\I'''$ be the instance for $\K''=(\T'',\DB')$ obtained by replacing in $\I'$ of Example~\ref{ex:interpretation} the equivalence class $[\Doe_1,\Doe_2,\Doe_4]$ with $[\Doe_1,\Doe_2,\Doe_4,\textnormal{\textbf{e}}_1^\bot]$, and by adding the facts $\CEO([\Yahoo],[\Doe_1,\Doe_2,\Doe_4,\textnormal{\textbf{e}}_1^\bot])$ and $\CEO([\IBM],[\textnormal{\textbf{e}}_2^\bot])$, $\Pers([\textnormal{\textbf{e}}_2^\bot])$.\nb{$\textnormal{\textbf{e}}_1^\bot$ will never added by a chase step, but it is true that $\I''$ is an instance (which is also a solution); the second rule saying that there is only one CEO for a company seems useless}
%%
Consider finally the following query asking for the CEOs:
\begin{equation}
\label{eq:query-CEO}
	q(x) \leftarrow CEO(z,x)
\end{equation}
\noindent We have that $q^{\I^{'''}} = \{ \tup{[\Doe_1, \Doe_2, \Doe_4,\textnormal{\textbf{e}}_1^\bot]}, \tup{[\textnormal{\textbf{e}}_2^\bot]} \}$, where the first and second answers are obtained through assignments $\mu''$ and $\mu'''$, respectively, %from $q(x)$ to $\I^{'''}$
defined as follows
\[
\begin{array}{lcl}
	\mu''(x)&=&[\Doe_1, \Doe_2, \Doe_4, \textnormal{\textbf{e}}_1^\bot]\\
	\mu''(z)&=&[\mathbf{\Yahoo}]\\
	\mu^{'''}(x)&=&[\textnormal{\textbf{e}}_2^\bot]\\
	\mu^{'''}(z)&=&[\mathbf{\IBM}]\\
\end{array}
\]
\qed
\end{example}

The following proposition follows from the definitions of answer to a query over an instance, 
%answer to a query, 
assignment, and homomorphism between instances. Intuitively, the proposition below clarifies how in our framework CQ answering is preserved under homomorphism.
%, and the fact that the composition of homomorphism with an assignment yields an assignment.
% this last property is not completely precise: composition of homomorphism with an assignment does not get and assignement, because the set you obtain is only required to be a subset of a set of entities or values in the instance $\I_2$. So it would be better to say something as follows
%
%\begin{proposition}
%    Given a KB $\K$, a conjunction of atoms $\phi(\vec{x})$, two instances for $\K$, $\I_1$ and $\I_2$, such that there is homomorphism $h$ from $\I_1$ to $\I_2$ and there is an assignment $\mu$ from $\phi(\vec{x})$ to $\I_1$. Then, there is and assignment $\mu'$ from $\phi(\vec{x})$ to $\I_2$. 
%    \end{proposition}
%    The assignment $\mu'$ is obtained by mapping a variable (or value) in $\phi(\vec{x})$ to the set $E$ such that $h(\mu(x)) \subseteq E$. %% THIS PROPOSITION IS NOT SUFFICIENTLY PRECISE



\begin{proposition}
	\label{pro:query-under-homo}
	Let $\K$ be a KB, $\I_1$ and $\I_2$ be two instances for $\K$, let $h:\I_1 \rightarrow \I_2$ be an homomorphism from $\I_1$ to $\I_2$, and let $q$ be a CQ. %of arity $n$. %The following holds
%	\begin{itemize}
%	\item if $q$ is Boolean and $\I_1 \models q$, then $\I_2 \models q$;
%	\item if $q$ is non-Boolean and if
 Then, for every $\vec{\genericSet} \in q^{\I_1}$ there is $\vec{\genericSettwo} \in q^{\I_2}$ such that $h(\vec{\genericSet}) \leq \vec{\genericSettwo}$.
 %% old (before def 10)
 %%  for every $\tup{\genericSet_1,\ldots,\genericSet_n} \in q^{\I_1}$ there is $\tup{\genericSettwo_1,\ldots,\genericSettwo_n} \in q^{\I_2}$ such that $h(\genericSet_i)  \subseteq \genericSettwo_i$, for each $1 \leq i \leq n$
%	\end{itemize}
\end{proposition}

\begin{proof}
	
Without loss of generality, let us consider the query $q(x,y)$ defined has $\exists w \, P_1(x,y,e) \land P_2(x,y,w,v)$, where $x$ is an entity-variable, $y$ and $w$ are value-variables, $e$ is an entity from $\alphaEntities$ and $v$ is a value from $\alphaValues$. By applying the $\tau$ operator to (the conjunction of atoms in) $q(x,y)$ we get $P_1(x,S_1^y,e) \land P_2(x,S_2^y,S^w,v)$. Then, by the definition of answer to a query over an instance it follows that for every tuple $\tup{E,V} \in q^{\I_1}$ there is an assignment $\mu$ from $q(x,y)$ to $\I_1$ such that, $\mu(x)=E$, $\mu(S_1^y)=V_1$, $\mu(S_2^y)=V_2$, $\mu(S^w)=V_3$, $\mu(v)=V_4$, $V=V_1 \cap V_2 =\emptyset$, $v \in V_4$, and $\I_1$ contains the facts $P_1(E,V_1,[e]_{\sim^1})$ and $P_2(E,V_2,V_3,V_4)$ (where $\sim^1$ is the equivalence relation associated to $\I_1$). Since $h$ is homomorphism from $\I_1$ to $\I_2$, the instance $\I_2$ has to contain the facts $P_1(\hat{E},\hat{V}_1,\hat{E}_1)$ and $P_2(\hat{E},\hat{V}_2,\hat{V}_3,\hat{V}_4)$, such that $P_1(h(E),h(V_1),h([e]_{\sim^1})) \leq P_1(\hat{E},\hat{V}_1,\hat{E}_1)$ and $P_2(h(E),h(V_2),h(V_3),h(V_4)) \leq P_2(\hat{E},\hat{V}_2,\hat{V}_3,\hat{V}_4)$
%%
%% alternative (no Definition 10)
%%
%%$h(E) \subseteq \hat{E}$, $h(V_1) \subseteq \hat{V}_1$, $h([e]_{\sim^1}) \subseteq \hat{E}_1$, $h(V_2) \subseteq \hat{V}_2$, $h(V_3) \subseteq \hat{V}_3$, and $h(V_4) \subseteq \hat{V}_4$.
%%
We then construct a mapping $\mu'$ from the variables and values in $P_1(x,S_1^y,e) \land P_2(x,S_2^y,S^w,v)$ to $\activeD_E(\I_2)$ as follows: $\mu'(x)=\hat{E}$, $\mu'(S_1^y)=\hat{V}_1$, $\mu'(S_2^y)=\hat{V}_2$, $\mu'(S^w)=\hat{V}_3$, and $\mu'(v)=\hat{V}_4$. It is not difficult to see that $\mu'$ is an assignment from $q(x,y)$ to $\I_2$. In particular: 
\begin{itemize}
\item since $e \in [e]_{\sim^1}$ and $h(e)=e$, then $e \in h([e]_{\sim^1})$, and since $h([e]_{\sim^1}) \subseteq \hat{E}_1$, it follows that $e \in \hat{E}_1$, which implies that $\hat{E}_1=[e]_{\sim^2}$ (where $\sim^2$ is the equivalence relation associated to $\I_2$);
\item since $V_1 \cap V_2 \neq \emptyset$ and since $h(V_1 \cap V_2) \subseteq h(V_1) \cap h(V_2) \subseteq \hat{V}_1 \cap \hat{V}_2$, it follows that that $\hat{V}_1 \cap \hat{V}_2 \neq \emptyset$;
\item since $v \in V_4$ and $h(v)=v$, then $v \in h(V_4)$, and since $h(V_4) \subseteq \hat{V}_4$, it follows that $v \in \hat{V}_4$.
\end{itemize}
The above assignment $\mu'$ testifies that $\tup{\hat{E},\hat{V}} \in q^{\I_2}$, where $\hat{V}=\hat{V}_1 \cap \hat{V}_2$. This proves the thesis, since, as said, $h(E) \subseteq \hat{E}$ and $h(V) \subseteq \hat{V}$.
	\end{proof}


%%In order to provide the definition of certain answers to a query over a KB we give some preliminary notions. 
%%
%%
%%\begin{definition}[answer tuple]
%%	\label{def:typed-tuple}
%%An \emph{answer tuple} is a sequence $\tup{T_1,\ldots,T_n}$, such that each $T_i$ is either a non-empty set of entities in $\alphaEntities$ or a non-empty set of values in $\alphaValues$.
%%\end{definition}

% commented because of the introduction of Definition~\ref{def:contain}
%
%Let $\vec{\genericSet} = \langle \genericSet_1, \dots, \genericSet_n \rangle$ and  $\vec{\genericSet'} = \langle \genericSet'_1, \dots, \genericSet'_n \rangle$ be two answer tuples, 
%we say that $\vec{\genericSet}$ and $\vec{\genericSet'}$ are \emph{equal}, denoted $\vec{T}=\vec{T'}$, if $\genericSet_i = \genericSet'_i$ for every $1 \leq i \leq n$. We also say that $\vec{\genericSet'}$ \emph{dominates} $\vec{\genericSet}$ (or analogously that $\vec{\genericSet}$ is dominated by $\vec{\genericSet'}$), denoted $\vec{\genericSet} \leq \vec{\genericSet'}$, if $\genericSet_i \subseteq \genericSet'_i$  for every $1 \leq i \leq n$. If  $\vec{\genericSet} \leq \vec{\genericSet'}$ and $\vec{\genericSet} \neq \vec{\genericSet'}$, we say that $\vec{\genericSet'}$ \emph{strictly dominates} $\vec{\genericSet}$, and denote it $\vec{\genericSet} < \vec{\genericSet}'$. We call the above order $\leq$ answer tuple dominance.

When querying a KB, we are interested in reasoning over all solutions of the KB. We thus adapt below the classical notion of certain answers to our framework. In the following, we say that a tuple $\vec{\genericSet} = \tup{\genericSet_1,\ldots,\genericSet_n}$ is  \emph{null-free} if $\genericSet_i \neq \emptyset$ and either $\genericSet_i \subseteq \alphaEntities$ or $\genericSet_i \subseteq \alphaValues$, for each $1 \leq i \leq n$ (that is, each $T_i$ is non-empty and does not contain nulls). 


\begin{definition}[certain answer]
	\label{def:certain-answer}
		Let $\K$ be a KB and $q$ a CQ. %of arity $n$. 
        An null-free tuple $\vec{T}$ %$\vec{T}=\langle T_1, \dots , T_n \rangle$ 
        is a \emph{certain answer} to $q$ \wrt $\K$ if:
	\begin{itemize}
		\item[($i$)]  for every $\I \in \Mod(\K)$ there exists a tuple %$\langle T'_1, \dots , T'_n \rangle \in q^\I$ such that $T_i \subseteq T'_i$, for each $1 \leq i \leq n$;
        $\vec{T'} \in q^{\I}$ such that $\vec{T} \leq \vec{T'}$;
		\item[($ii$)]   there is no null-free tuple $\vec{T'}$ that satisfies ($i$)  such that $\vec{T} < \vec{T'}$.
	\end{itemize}
The set of certain answers to $q$ \wrt $\K$ is denoted by $\cert(q,\K)$.
\end{definition}



Note that Condition~$(ii)$ in the above definition says that a certain answer has to be a maximal null-free tuple with respect to the tuple dominance order $\leq$ given in Definition~\ref{def:contain}, among the tuples satisfying Condition~$(i)$. The following example clarifies the importance of this condition.

% \begin{example}
% 	Consider a KB $\K$ whose database is constituted by the facts $has\_name(\Doe_1,\texttt{J.Doe})$ and $has\_name(\Doe_2, \texttt{J.Doe})$, and whose TBox is constituted by the entity-egd $has\_name(x_1,y),has\_name(x_2,y) \ra x_1=x_2$.
% 	It is easy to see that, in every solution for $\K$, $\Doe_1$ and  $\Doe_2$ must belong to the same equivalence class, and that the (unary) answer tuple $\tup{\{\Doe_1,\Doe_2\}}$ is a certain answer to the query $q(x) \la has\_name(x,y)$. The answer tuple $\tup{\{\Doe_1\}}$ instead is not a certain answer, even if it satisfies condition $(i)$  of Definition~\ref{def:certain-answer}, since it does not respect condition $(ii)$  (analogously for the answer tuple $\tup{\{\Doe_2\}}$).
	
% 	\qed
% \end{example}

\begin{example}
	Consider the setting in the Example~\ref{ex:query}. It is easy to see that, in every solution for $\K''$, $\Doe_1$, $\Doe_2$, and $\Doe_4$ must belong to the same equivalence class, and that such class must denote a CEO. %(i.e., an antity occurring as second component of the $\CEO$ predicate). 
    Then, the (unary) null-free tuple $\tup{\{\Doe_1,\Doe_2,\Doe_4\}}$ is a certain answer to query~(\ref{eq:query-CEO}). Notice however that also, e.g., the null-free tuple $\tup{\{\Doe_1\}}$ satisfies Condition $(i)$  of Definition~\ref{def:certain-answer}, but it is not a certain answer since it does not respect Condition $(ii)$.  \qed
\end{example}

The following properties tell us that %the set of certain answers to a query $q$ is such that 
if two sets of entities appear in the same or in different certain answers, They are the same set or are disjoint. In particular, we can identify the sets of entities that appear in the set of certain answers with the equivalence classes of some equivalence relation.

 
\begin{proposition}
	\label{pro:partition-of-certain-answers}
	Let $\K$ be a KB, $q$ be a CQ of arity $n$, $\vec{\genericSet}=\langle T_1, \dots , T_n \rangle$ and $\vec{\genericSet'}=\langle T'_1, \dots, T'_n \rangle$ be two certain answers to $q$ \wrt $\K$. If $T_i$ and $T'_j$ are sets of entities, then either $T_i = T'_j$ or $T_i \cap T'_j = \emptyset$, for any $1\leq i,j\leq n$.
\end{proposition}

\begin{proof}
	Towards a contradiction, assume that $T_i$, $T'_j$ are two non-empty sets of entities such that $T_i \neq T'_j$ and $T_i \cap T'_j \neq\emptyset$. Then $T_i \subsetneqq T_i \cup T'_j$ or $T'_j \subsetneqq T_i \cup T'_j$. Let's assume $T_i \subsetneqq T_i \cup T'_j$. Since $\langle T_1, \dots, T_n \rangle$ and $\langle T'_1, \dots, T'_n \rangle$ are certain answers of $q$, for every solution $\I$, there are tuples $\langle L_1, \dots, L_n \rangle$, $\langle L'_1, \dots, L'_n \rangle$ in $q^\I$ such that for every $k$ we have $T_k \subseteq L_k$ and $T'_k \subseteq L'_k$. Thus we have that $T_i \subseteq L_i$ and $T'_j \subseteq L'_j$. Since $T_i \cap T'_j \neq \emptyset$, it follows that $L_i \cap L'_j \neq \emptyset$. However, $L_i$, $L'_j$ are equivalence classes in the solution $\I$, hence they must coincide, i.e. $L_i = L'_j$. It follows that $T_i \cup T'_j \subseteq L_i = L'_j$. Consider now the tuple $\langle T_1, \dots, T_{i-1}, T_i \cup T_j ,T_{i+1}, \dots ,T_n \rangle$, which is obtained from $\langle T_1, \dots, T_n \rangle$ by replacing $T_i$ by $T_i \cup T_j$. Note that $\langle T_1, \dots, T_{i-1}, T_i ,T_{i+1}, \dots ,T_n \rangle < \langle T_1, \dots, T_{i-1}, T_i \cup T_j ,T_{i+1}, \dots ,T_n \rangle$ because $T_i \subsetneqq T_i \cup T'_j$. However for every solution $\I$ of $\K$, we have that $T_i \cup T'_j \subseteq L_i$, and for all $1 \leq k \leq n$ such that $k \neq i$, we have that $T_k \subseteq L_k$. This means that $\langle T_1, \dots, T_{i-1}, T_i \cup T_j ,T_{i+1}, \dots ,T_n \rangle$ satisfies Condition~$(i)$ of Definition~\ref{def:certain-answer}, and therefore $\langle T_1, \dots, T_n \rangle$ does not respect Condition~$(ii)$ of Definition~\ref{def:certain-answer}), and thus it is not a certain answer, which is a contradiction. Note finally that if we assume $T'_j \subsetneqq T_i \cup T'_j$ we contradict that $\langle T'_1, \dots, T'_n \rangle$ is a certain answer by using an analogous argument. 
\end{proof}


%%The following property easily follows from the above proposition.

\begin{corollary}
	\label{cor:partition-of-certain-answers}
	Let $\K$ be a KB, $q$ be a CQ, and %$\vec{\genericSet}=$ 
	$\langle T_1, \dots ,T_n \rangle$ be %a typed tuple. If $\vec{t}$ is 
	a certain answer to $q$ with respect to $\K$. If $T_i$ and $T_j$ are set of entities %occurring in $\vec{t}$ 
	such that $i \neq j$, then either $T_i = T_j$ or $T_i \cap T_j$.
\end{corollary}

\begin{proof}
	%The thesis 
 It follows from Proposition~\ref{pro:partition-of-certain-answers} when $\vec{T}=\vec{T'}$. 
\end{proof}



We now explain the relation existing between universal solutions and certain answers. To this aim, we have to introduce an operator, denoted $\downarrow$,  that suitably allows us to get rid of entity-nulls and value-nulls when evaluating a query over an instance of a KB (analogously to what is done in the context of Data Exchange~\cite{FKMP05}). Formally, let $\entitySet$ be a set of entities and entity-nulls and $\valueSet$ be a non-empty set of values and value-nulls, $\entitySet\downarrow=\{e~|~e \in \alphaEntities \cap \entitySet\}$ and  $\valueSet\downarrow=\{v~|~v \in \alphaValues \cap \valueSet\}$, i.e., $\downarrow$ removes from $\entitySet$ and from $\valueSet$ all nulls. Then, let $\langle T_1, \dots,T_n \rangle$ be a tuple such that each $T_i$ is either a set of entities and entity-nulls or a set of values and value-nulls, we have that $\langle T_1, \dots,T_n \rangle{\downarrow} = \langle T_1 {\downarrow}, \dots,T_n {\downarrow} \rangle$.
%%
Finally, given a set $\Theta$ of tuples of the form above,
%of the form $\langle T_1, \dots,T_n \rangle$, where each $T_i$ is either a set of entities and entity-nulls, or  a set of values or value-nulls, 
$\Theta {\downarrow}$ is the set obtained from $\Theta$ by removing all tuples in $\Theta$ containing a $T_i$ such that $T_i {\downarrow} = \emptyset$, and replacing each other tuple $\langle T_1, \dots,T_n \rangle$ in $\Theta$ by the tuple $\langle T_1, \dots,T_n \rangle {\downarrow}$.

Whereas under standard semantics, for several tractable ontology languages, %(typically equivalent to special sets of tgds and egds), 
the set of certain answers to a CQ $q$ can be obtained by first computing the answers to $q$ over a universal solution and then filtering such answers through the $\downarrow$ operator (see, e.g., ~\cite{FKMP05,CDLLR07}), in our framework this is not the case, as shown by the example below.

\begin{example}
Let $P_1$ and $P_2$ be binary predicates such that $\type(P_1)=\type(P_2)=\tup{\entity,\val}$. Consider the KB $\K=\tup{\T,\DB}$, such that $\T$ is constituted by the following rules
$$
	\begin{array}{l}
	P_1(x,y) \rightarrow P_2(x,y)\\
	P_1(x,y) \land P_1(x,z) \rightarrow y=z
\end{array}
$$
and $\DB=\{P_1(\textnormal{\textbf{e}},1), P_1(\textnormal{\textbf{e}},2)\}$.
%
Consider then the following universal solutions for $\K$
$$
\begin{array}{lcl}
\I_1 &=& \{P_1([\textnormal{\textbf{e}}],\{1,2\}), P_2([\textnormal{\textbf{e}}],\{1,2\})\}\\
\I_2 &=& \{P_1([\textnormal{\textbf{e}}],\{1,2\}), P_2([\textnormal{\textbf{e}}],\{1\}), P_2([\textnormal{\textbf{e}}],\{1,2\})\}
\end{array}
$$
and the query $q(x,y):-P_2(x,y)$.
We have that:
$q^{I_1}=\{\tup{[\textnormal{\textbf{e}}],\{1,2\}}\}$, and $q^{\I_2}=\{\tup{[\textnormal{\textbf{e}}],\{1,2\}}, \tup{[\textnormal{\textbf{e}}],\{1\}}\}$. In particular, $q^{\I_2}$ does not coincide with the set of certain answers, because the tuple $\tup{[\textnormal{\textbf{e}}],\{1\}}$ does not satisfy Condition $(ii)$ of Definition~\ref{def:certain-answer}.
\qed
	\end{example}


%\begin{example}
%	Let $A1,A2,A3$ be binary predicates such that $\type(Ai)=\tup{\entity,\val}$,for each $Ai$. Consider the following KB\nb{put a better example}
%	\begin{verbatim}
%		A1(x,y) -> A2(x,y)
%		A3(x,y) -> A2(x,y)
%		A3(x,y),A3(x,z) -> y=z 
%		A1(e,1),
%		A3(e,1),
%		A3(e,2)
%	\end{verbatim}
%	and the following universal solutions, $\I_1$ and $\I_2$
%	\begin{verbatim}
%		A1([e],{1}), A2([e],{1}), A3([e],{1,2}), A2([e],{1,2})
%		A1([e],{1}), A3([e],{1,2}), A2([e],{1,2})
%	\end{verbatim}
%	and the query $q(x,y):-A2(x,y)$.
%	We have that:
%	$q^{I_1}=\{\tup{[e],\{1,2\}}, \tup{[e],\{1\}}\}$, and $q^{I_2}=\{\tup{[e],\{1,2\}}\}$.
%\end{example}

Intuitively, in the above example the universal solution $\I_2$ is not ``minimal'', in the sense that the fact 
$P_2([\textnormal{\textbf{e}}],\{1\})$ in $\I_2$ is dominated by another fact of $\I_2$, namely $P_2([\textnormal{\textbf{e}}],\{1,2\})$. %Thus, the fact $P_2([e],\{1\})$ is somehow useless for the computation of the certain answers, but still occurs in the universal solution $\I_2$, 
This behaviour causes that that the answer to the query over $\I_2$ contains also tuples that are not maximal with respect to tuple dominance (cf.\ Definition~\ref{def:certain-answer}). Notice also that in the presence of nulls the situation is even slightly more complicated. For example, we might have an instance containing both facts $Q([\textnormal{\textbf{e}}],\{1,2,n\})$ and $Q([\textnormal{\textbf{e}}],\{1,n'\})$, where $n$ and $n'$ are two different value-nulls. In this case, no fact in the solution is dominated by another fact, still the phenomenon shows up if we eliminate the nulls. This suggests that we need some additional processing after we get rid of the nulls. To this aim, we modify the $\downarrow$ operator by performing a further ``reduce'' step. The new operator is denoted $\dareduced$ and is defined as follows. Given a query $q$ and an instance $\I$ for a KB $\K$, we write $q^\I\dareduced$ to denote the set of null-free tuples obtained through following three steps:
\begin{enumerate}
\item evaluate $q$ on $\I$ and obtain $q^\I$;
\item compute $q^\I\downarrow$;
\item remove from  $q^\I\downarrow$ all tuples strictly dominated by other tuples in the set, that is, if $\vec{\genericSet}$ and $\vec{\genericSet'}$ are two tuples in $q^\I\downarrow$ such that $\vec{\genericSet} < \vec{\genericSet'}$, then remove $\vec{\genericSet}$ from $q^\I\downarrow$.
%if $\tup{T_1,\ldots,T_k}$ and $\tup{T_1',\ldots,T_k'}$ are two tuples obtained in Step~2 such that $\tup{T_1',\ldots,T_k'}$  dominates $\tup{T_1,\ldots,T_k}$, then we remove $\tup{T_1,\ldots,T_k}$.
\end{enumerate}

%Esempio più complicato: Faccio vedere una universal solution, ma la valutazione della query q(x,y):-P(x,y) restituisce <[e],{1,2,n_1}>,<[e],{1,n_2}>; applico downarrow ed ottengo <[e],{1,2}>,<[e],{1}>; devo quindi applicare la reduce
%
%P_0(x,y),P_0(x,z)->y=z
%P_1(x,y),P_1(x,z)->y=z
%
%P_0(x,y)->P(x,y)
%P_1(x,y)->P(x,y)
%
%P_2(x)->P_3(x,y)
%P_3(x,y)->P_0(x,y)
%
%P_4(x)->P_5(x,y)
%P_5(x,y)->P_1(x,y)
%
%P_0(e,1)
%P_0(e,2)
%P_2(e)
%
%P_1(e,1)
%P_4(e)

The following property is needed to prove the last theorem of this section. It easily follows from Proposition~\ref{pro:query-under-homo} and Definition~\ref{def:homomorphism}.

% old: it is as the new version, but does not use \vec{T} and \vec{U}
%
%\begin{corollary}
%	\label{cor:query-over-univ-solution}
%	Let $\K$ be a KB, $q$ be a CQ of arity $n$, $\U$ be a universal solution for $\K$, and $\tup{\genericSet_1,\ldots,\genericSet_n} \in q^{\U}$. Then, for every $\I \in \Mod(\K)$ there is a tuple $\tup{\genericSettwo_1,\ldots,\genericSettwo_n} \in q^{\I}$ such that $\genericSet_i \downarrow \subseteq \genericSettwo_i \downarrow \subseteq \genericSettwo_i$, for each $1 \leq i \leq n$\nb{It seems that we do not really need $\genericSet_i \downarrow \subseteq \genericSettwo_i \downarrow$ (as in the Phokion's note), but $\genericSet_i \downarrow \subseteq \genericSettwo_i$ is enough.}.
%\end{corollary}
%\begin{proof}
%	Since $\U$ is universal, there is a homomorphism $h$ from $\U$ to $\I$. From Proposition~\ref{pro:query-under-homo} it follows that there is $\tup{\genericSettwo_1,\ldots,\genericSettwo_n} \in q^{\I}$ such that $h(\genericSet_i) \subseteq \genericSettwo_i$, for each $1 \leq i \leq n$. From Definition~\ref{def:homomorphism} (homomorphism) it follows that $\genericSet_i \downarrow \subseteq h(\genericSet_i)$, and thus $\genericSet_i \downarrow \subseteq \genericSettwo_i$. By applying the $\downarrow$ operator to $\genericSettwo_i$, we eliminate from $\genericSettwo_i$ only entity-nulls or value-nulls, which cannot be contained in $\genericSet_i \downarrow$. We can thus conclude that $\genericSet_i \downarrow \subseteq \genericSettwo_i \downarrow$, q.e.d.
%\end{proof}


\begin{corollary}
\label{cor:query-over-univ-solution}
Let $\K$ be a KB, $q$ be a CQ, $\U$ be a universal solution for $\K$, and $\vec{\genericSet} \in q^{\U}$. Then, for every $\I \in \Mod(\K)$ there is a tuple $\vec{\genericSet'} \in q^{\I}$ such that $\vec{\genericSet}\downarrow \leq \vec{\genericSet'}\downarrow \leq \vec{\genericSet'}$\nb{It seems that we do not really need $\vec{\genericSet}\downarrow \leq \vec{\genericSet'}\downarrow$ (as in the Phokion's note), but $\vec{\genericSet}\downarrow \leq \vec{\genericSet'}$ is enough.}.
\end{corollary}
\begin{proof} Obviously, $\vec{\genericSet'}\downarrow \leq \vec{\genericSet'}$.
Since $\U$ is universal, there is a homomorphism $h$ from $\U$ to $\I$. From Proposition~\ref{pro:query-under-homo} it follows that there is $\vec{\genericSet'} \in q^{\I}$ such that $h(\vec{\genericSet}) \leq \vec{\genericSet'}$. From Definition~\ref{def:homomorphism} (homomorphism) it follows that $\vec{\genericSet}\downarrow \leq h(\vec{\genericSet})$, and thus $\vec{\genericSet}\downarrow \leq \vec{\genericSet'}$. By applying the $\downarrow$ operator to $\vec{\genericSet'}$, we eliminate from the sets occurring in $\vec{\genericSet'}$ only entity-nulls or value-nulls, which cannot be contained in the sets occurring in $\vec{\genericSet} \downarrow$. We can thus conclude that $\vec{\genericSet} \downarrow \leq \vec{\genericSet'} \downarrow$.
\end{proof}
We are now in the condition to prove the main result of this section, which says how universal solutions can be exploited to compute the certain answers to a conjunctive query.

\begin{theorem}
	\label{ref:thm-query-answering}
	Let $\K$ be a KB, $q$ be a CQ, and $\U$ be a universal solution for $\K$. Then $\cert(q,\K) =  q^\U{{\dareduced}}$.
\end{theorem}

\begin{proof}
We first show that $q^\U{\dareduced} \subseteq \cert(q,\K)$. Let $\vec{\genericSet} \in {q^{\U}\dareduced}$, which of course implies $\vec{\genericSet} \in q^{\U}$. By Corollary~\ref{cor:query-over-univ-solution} we have that for every $\I \in \Mod(\K)$ there is a tuple $\vec{\genericSet'} \in q^{\I}$ such that $\vec{\genericSet}\downarrow \leq \vec{\genericSet'}$. Since $\vec{\genericSet} \in {q^{\U}\dareduced}$, it is null-free and thus $\vec{\genericSet}\downarrow=\vec{\genericSet}$. Hence, Condition~$(i)$ of Definition~\ref{def:certain-answer} (certain answers) is satisfied by $\vec{\genericSet}$. 
%%
Let us now assume by contradiction that $\vec{\genericSet}$ does not satisfy Condition~$(ii)$ of Definition~\ref{def:certain-answer}. This means that there exists a null-free tuple $\vec{\genericSet'}$ satisfying Condition~$(i)$ of Definition~\ref{def:certain-answer} such that $\vec{\genericSet} < \vec{\genericSet'}$. Since $\vec{\genericSet'}$ satisfies Condition~$(i)$ of Definition~\ref{def:certain-answer}, there must exist a tuple $\vec{\genericSettwo} \in q^\U$ such that $\vec{\genericSet'} \leq \vec{\genericSettwo}$, and thus obviously $\vec{\genericSet} < \vec{\genericSettwo}$. We can apply the $\downarrow$ operator to both $\vec{\genericSet}$ and $\vec{\genericSettwo}$ and get $\vec{\genericSet}\downarrow < \vec{\genericSettwo}\downarrow$, and since, as said, $\vec{\genericSet}=\vec{\genericSet}\downarrow$, we have that $\vec{\genericSet}< \vec{\genericSettwo}\downarrow$, which is a contradiction. Indeed, $\vec{\genericSet} \in q^{\U}\dareduced$ (by hypothesis) and $\vec{\genericSettwo}\downarrow \in q^{\U}\downarrow$, and thus it is not possible that $\vec{\genericSettwo}$ dominates $\vec{\genericSet}$ (cf.\ Step~3 of the definition of the $\dareduced$ operator). 

We now show that $\cert(q,\K)\subseteq q^\U{\dareduced}$. Let $\vec{\genericSet} \in \cert(q,\K)$. By Condition~$(i)$ of Definition~\ref{def:certain-answer} there exists a tuple $\vec{\genericSettwo} \in q^\U$ such that $\vec{\genericSet} \leq \vec{\genericSettwo}$, which implies $\vec{\genericSet} \leq \vec{\genericSettwo}\downarrow$ (since $\vec{\genericSet}$ is null-free). %We now show that in fact $\vec{\genericSet} = \vec{\genericSettwo}\downarrow$, which implies that $\vec{\genericSet} \in q^\U\downarrow$. 
By Corollary~\ref{cor:query-over-univ-solution}, we have that for each $\I \in \Mod(\K)$ there is a tuple $\vec{\genericSet'} \in q^{\I}$ such that $\vec{\genericSettwo} \downarrow \leq \vec{\genericSet'}$. This last fact implies that $\vec{\genericSettwo} \downarrow $ is a null-free tuple satisfying Condition~$(i)$ of Definition~\ref{def:certain-answer}. Thus, if $\vec{\genericSet} < \vec{\genericSettwo}\downarrow$ then $\vec{\genericSet}$ is not a certain answer, which contradicts the assumption. Therefore, it must be $\vec{\genericSet} = \vec{\genericSettwo}\downarrow$. This shows that $\vec{\genericSet} \in q^\U\downarrow$. Let us assume by contradiction that $\vec{\genericSet} \not \in q^\U\dareduced$. By definition of the $\dareduced$ operator, the above assumption implies that there exists a tuple $\vec{X} \in q^\U\dareduced$ such that $\vec{T} < \vec{X}$, and since $q^\U\dareduced \subseteq \cert(q,\K)$, as shown in the first part of this proof, $\vec{X}$ satisfies Condition~$(i)$ of Definition~\ref{def:certain-answer}, which in turn implies that $\vec{T} \not \in \cert(q,\K)$, which is a contradiction.
%Then, By Condition~$(ii)$ of Definition~\ref{def:certain-answer} it follows that $\vec{\genericSet}$ is maximal w.r.t.\ tuple domination, which implies that $\vec{\genericSet}\in q^\U\dareduced$.
\end{proof}

\begin{example}
    Consider the setting in the Example~\ref{ex:query}. It is easy to see that $\I^{'''}$ is an universal solution for $\K''$. Then $\cert(q,\K'') = \{ \tup{[\Doe_1,\Doe_2,\Doe_4]}\}$ 
\end{example}





==> 06-Computing_Universal_Model/computing-federico.tex <==
\newcommand{\facts}{\mathrm{Facts}}
\newcommand{\factSequence}{\mathrm{FactDerivation}}
\newcommand{\limit}{\mathit{lim}}
\newcommand{\pred}{\mathit{Pred}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vx}{\vec{x}}


\section{Computing a universal model}
\label{sec:computing-Univ-Model}

In the following we adapt the well-known notion of restricted chase~\cite{BeVa84,JoKl84,FKMP05,CDLLR07}
to our framework. Intuitively, given a KB $\K=\tup{\T,\DB} $, to chase $\K$ we define a procedure that starts from an instance for $\K$ ``specular'' to the database $\DB$, which we call the base instance of $\DB$, and incrementally constructs an instance that satisfies the tgds and the edgs of the TBox $\T$. This is obtained by iteratively applying three chase rules, one for each kind of rule that may occur in $\T$, as long as they are triggered in the (current) instance.
Interestingly, the chase procedure we define never produces a failure, 
%caused by the presence of and entity resolution rules, 
as, e.g., for the application  egds in the chase rules described in \cite{FKMP05}, since different entities occurring in a database %have not to be considered hard-constants, which cannot be made equal, but rather are soft-constants that 
can be gathered together within the same equivalence class, when an entity-egd imposes such entites to be the same. %(which means that they are denoting the same object of the world). 
Similarly, we never say that an equality between different values imposed by a value-egd produces a failure, rather, we take the union of such values and modify the instance accordingly.  
%\todo{This is however not true if we allow for negative inclusions, i.e., forms of disjointness between classes or roles, as in $\dllitea$}. 
However, because of the presence of cycles among the tgds of the TBox, it is possible that chase rule application may continue indefinitely, that is, the chase procedure has infinitely many steps, each producing a new instance. As a consequence, some care is required in defining the result of the application of this (potentially infinite) procedure to a KB $\K$, so that we can obtain an instance that can be used (at least in principle) for query answering. We call such instance \emph{the result of the chase of the KB $\K$}, and distinguish the case in which the chase terminates from the case in which it does not. In the former situation, the result of the chase of $\K$ is simply the instance produced in the last step of the chase sequence, and we show that it is indeed a universal solution for $\K$. For the latter case we show that previous approaches from the literature for infinite standard chase sequences under tgds and egds cannot be smoothly adapted to our framework, and we leave it open how to define the result of the chase for infinite chase sequences so that it is a universal solution.
%For the latter case, we propose a novel notion of result of the chase, which we are able to prove it is a solution for $\K$, and which we conjecture is also universal.

%Whereas for the finite case the chase procedure provides directly an algorithm for query answering, for the infinite case it seems that it is useless for this purpose. Nonetheless, there is then room to study whether, at least in some cases of practical interest, there are finite representations of the chase that can be used for query answering, maybe for certain classes of Conjunctive Queries, or it can be used as a theoretical tool useful to identify query rewriting algorithms, as in~\cite{CDLLR07,BiOr15,other}.
%i.e., mechanisms that reformulate the input query so that its certain answers can be obtained by evaluating such reformulation over the database $\DB$, in the spirit of the works on query answering using views or ontology-mediated query answering~\cite{CDLLR07,BiOr15}.

We start with the notion of base instance for a database. 
%
% old - base interpretation
%
%\begin{definition}[base interpretation for a database]
%	\label{def:minimal-abox-model}
%	Let $\DB$ be a database, the \emph{base interpretation for $\DB$} is the interpretation $\I^\DB = \langle \Delta^{\I^\DB}, \sim^{\I^\DB}, \cdot^{\I^\DB} \rangle$, such that:
%	\begin{itemize}
%		\item $\Delta^{\I^\DB}=\Delta^{\I^\DB}_E \cup \Delta^{\I^\DB}_V$, where $\Delta^{\I^\DB}_E=\mathsf{N_E}$ and $\Delta^{\I^\DB}_V=\mathsf{N_V}$;
%		\item $\sim^{\I^\DB} = \{ \langle e, e \rangle \mid e \in \Delta^{\I^\DB}_E \}$;
%		\item $e^{\I^\DB} = \{e\}$ %[e]^{\sim^{\I^\DB}}$, 
%		for each entity $e \in \Delta^{\I^\DB}_E $; %occurring in $\DB$;
%		\item $v^{\I^\DB} = v$, for each value $v \in \Delta^{\I^\DB}_V $; %occurring in $\DB$;
%		\item for each $n$-ary predicate $P$ occurring in $\DB$, $P^{\I^\DB}$ is the set of tuples $\tup{\genericSet_i,\ldots,\genericSet_n}$ such that there exists $P(c_1,\ldots,c_n) \in \DB$ and, for $1 \leq i \leq n$, it holds either $\genericSet_i=[c_i]^{\sim^{\I^\DB}}$, if $\type(P,i)=\entity$,  or $\genericSet_i=\{c_i\}$, if $\type(P,i)=\val$. 
%	\end{itemize}	
%\end{definition}
%
%
%It is easy to see that $\I^\DB$ is well-defined, i.e., $\I^\DB$ is indeed an interpretation (in particular $[e]^{\sim^{\I^\DB}}=\{e\}$ for every $e \in \Delta^{\I^\DB}_E $), and that it is a model of $\tup{\emptyset,\DB}$, (for simplicity, we may also say that $\I^\DB$ is a model for $\DB$) .
%
%Note that the elements in $\Delta^{\I^\DB}_E/{\sim^{\I^\DB}} $ are singletons because $\sim^{\I^\DB} $ contains only pairs of entities equal only to themselves.
%
Given a database $\DB$, we define the set 
$$\I^{\DB}=\{P(\{c_1\},\ldots,\{c_n\})~|~P(c_1,\ldots,c_n) \in \DB\}$$ 
It is easy to see that $\I^{\DB}$ is an instance for $(\emptyset,\DB)$ \wrt the identity relation $\id$ over the set $\S=\alphaEntities \cap \sig((\emptyset,\DB))$. We call $\I^\DB$ the \emph{base instance} for  $(\emptyset,\DB)$ (or simply for $\DB$).
%
Note that a base instance for $\DB$ is also a solution for $(\emptyset,\DB)$ (again, we may simply say for $\DB$).


We next define three chase steps, one for tgds, one for entity-egds, and one for value-egds. 

% The following is wrong: wehave then decided to not impose any order but assume that one well-defined order does exist that ensure no-starvation and can be chosen
%
%\nb{The definition of order does not work. See next comment. This part has to be revised}It is convenient to define a total order on all the predicates, entities, values, labeled nulls, variables, and symbols used in tgds, egds, and images of assignments.
%%%
%From $\entitynulls = \{ e_{1{\bot}}, e_{2{\bot}}, \dots \}$ and $\valuenulls = \{ v_{1{\bot}}, v_{2{\bot}} \dots \}$, we define $\Delta_{{EV}_\bot}$ as the sequence  $ e_{1{\bot}}, v_{1{\bot}}, e_{2{\bot}}, v_{2{\bot}}, \dots$, i.e., the ordered list obtained by alternating the elements of $\entitynulls$ with those of $\valuenulls$ (without selecting twice the same element). 
%We can now consider the set $\A=\alphaPredicates  \cup \alphaBuiltIns \cup \alphaEntities \cup \alphaValues \cup \{\forall,\exists,~.,(,~),~\land,~,\},\{,],[~\}\cup \alphaVariables$ %$\cup \Delta_{{VE}_\bot}$,
%%%\cup \{\land \rightarrow \sim \exists , )\}
%and define a total order on $\A$ and on the sequence $\Delta_{{EV}_\bot}$, such that all the elements in  $\Delta_{{EV}_\bot}$ follows, in the same order they have in  $\Delta_{{EV}_\bot}$ , all the other elements of $\A$.
%%The order defined above induces a lexicographic order on tgds and entity resolution rules.
%
%We now define an order over assignments to an interpretation $\I$ whose domain $\Delta^{\I}=\Delta^\I_{E} \cup \Delta^\I_{V}$ is such that $\Delta^\I_E \setminus \mathsf{N_E} \subseteq \Delta_{E_\bot}$ and $\Delta^\I_V \setminus \mathsf{N_V} \subseteq \Delta_{V_\bot}$.  
%% OLD - IT IS USELESS
%%To this aim, we represent every equivalence class $\entitySet$ (resp.\ sets $\valueSet$ of values) in the image of an assignment $\mu$ as the string obtained by concatenating all the elements occurring in $\entitySet$ (resp.\ $\valueSet$), following the order defined above. As a consequence, the entire image can be represented as a string. 
%Specifically, given an assignment $\mu$ from a conjunction of atoms $\phi$ to $\I$ and an assignment $\mu'$ from a conjunction of atoms $\phi'$ to $\I$,  we say that \emph{$\mu$ precedes $\mu'$} if $(i)$
%$\mu(\phi)$ precedes lexicographically $\mu'(\phi')$, where $\desc$ is a function that takes as input a string $s$ and returns a string $s'$ containing exactly the same symbols in $s$ but put in descending order or $(ii)$ if $\mu(\phi)=\mu'(\phi')$
%%$\desc(\mu(\phi))$ precedes lexicographically $\desc(\mu'(\phi'))$, where $\desc$ is a function that takes as input a string $s$ and returns a string $s'$ containing exactly the same symbols in $s$ but put in descending order or $(ii)$ if $\desc(\mu(\phi))=\desc(\mu'(\phi'))$ 
%(i.e., $\mu(\phi)$ and $\mu'(\phi')$ are the same string), $\phi$ precedes $\phi'$. 
%%%
%Notice that we always have  that either $\mu$ precedes $\mu'$ or  $\mu'$ precedes $\mu$, unless $\phi=\phi'$ and $\mu(\phi)=\mu'(\phi')$.
%%%
%Hereinafter, we also assume that the variables occurring in a rule (tgd or egd) of a KB $\K$ are different from the variables used in all the other rules of $\K$. This assumption implies that for any two assignments $\mu$ and $\mu'$ from the body of two different rules $r$ and $'r$ in $\K$ it always holds that $\mu$ precedes $\mu'$ or viceversa.\nb{This property is true, but does not solve the problem we have: all assignments from the body of A(x,y)->A(y,z) will always precede assignments from the body of B(x)->C(x), and thus a chase for a DB={A(c,d) B(c)} will never apply B(x)->C(x) to B(d)}

% OLD: uses intepretations (and orders)
%
%We are now ready to give the definition of chase step.
%
%\begin{definition}[Chase Step] 
%	\label{def:chaseStep}	
%	Let $\I_1=(\Delta^{\I_1},\sim^{\I_1},\cdot^{\I_1})$, where $\Delta^{\I_1}=\Delta^{\I_1}_E \cup \Delta^{\I_1}_V$ and $\Delta^{\I_1}_E \cap \Delta^{\I_1}_V=\emptyset$, be an interpretation such that $\Delta^{\I_1}_E \setminus \mathsf{N_E} \subseteq \entitynulls$, and $\Delta^{\I_1}_V \setminus \mathsf{N_V} \subseteq \valuenulls$.
%	
%	%	and $\valuenulls$ and $\entitynulls$ be as defined above.
%	\begin{itemize}
%		\item (tgd) let $d$ be a tgd of the form (\ref{eq:tgd}). We denote with $\vec{y_e}=y_e^1,\ldots y_e^h$ and $\vec{y_v}=y_v^1,\ldots,y_v^j$ the entity-variables and value-variables in $\vec{y}$, respectively. Let $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$ such that there is no $\psi(\vec{x},\vec{y})$-compatible tgd-extension of  $\mu$ to $\I_1$. 
%		%%
%		We say that $d$ is applicable to $\I_1$ with assignment $\mu$ (or analogously that $\mu$ triggers $d$ in $\I_1$),	and	construct $\I_2=(\Delta^{\I_2},\sim^{\I_2}, \cdot^{\I_2})$ as follows:
%		\begin{itemize}
%			\item  $\Delta^{\I_2}=\Delta^{\I_2}_E \cup \Delta^{\I_2}_V$, such that $\Delta^{\I_2}_E=\Delta^{\I_1}_E \cup \Delta_{E_\bot}^{fresh}$ and $\Delta^{\I_2}_V=\Delta^{\I_1}_V \cup \Delta_{V_\bot}^{fresh}$, where %$\Delta_{E_\bot}^{fresh} \subseteq \Delta_{E_\bot}$,  $\Delta_{V_\bot}^{fresh} \subseteq \Delta_{V_\bot}$, $|\Delta_{E_\bot}^{fresh}|=|\vec{y_e}|$, $|\Delta_{V_\bot}^{fresh}|=|\vec{y_v}|$,
%			%and the nulls in  $\Delta_{E_\bot}^{fresh}$ and $\Delta_{V_\bot}^{fresh}$ are fresh symbols, not occurring in $\Delta^{\I_1}$ that follows (in the order) all the entity-nulls and value-nulls in $\Delta^{\I_1}$;
%			$\Delta_{E_\bot}^{fresh}=\{f_e^1,\ldots,f_e^h\} \subseteq \Delta_{E_\bot}$,  $\Delta_{V_\bot}^{fresh}=\{f_v^1,\ldots,f_v^j\} \subseteq \Delta_{V_\bot}$ are such that the elements they contain are fresh null symbols, i.e., not occurring in $\Delta^{\I_1}$, {\color{blue} that follows (in the order) all the entity-nulls and value-nulls in $\Delta^{\I_1}$};
%			\item $\sim^{\I_2}=\sim^{\I_1} \cup \{\tup{f_e,f_e} \mid f_e \textrm{ is a fresh entity-null in } \Delta_{E_\bot}^{fresh}\}$;
%			%			\item $e^{\I_2}=e^{\I_1}$ and $v^{\I_2}=v^{\I_1}$ for each entity $e \in \mathsf{N_E}$ and each value $v \in \mathsf{N_V}$;
%			\item $e^{\I_2}=e^{\I_1}$ and $v^{\I_2}=v^{\I_1}$ for each entity $e \in \alphaEntities$ and each value $v \in \alphaValues$, respectively;
%			\item $P^{\I_2}= P^{\I_1}$, for each predicate $P$ in $\alphaPredicates$ not occurring in $\psi(\vec{x},\vec{y})$;
%			\item for each predicate $P$ occurring in $\psi(\vec{x},\vec{y})$, proceed as follows:\\[2mm]
%			%%
%			\hspace*{0.2cm} $P^{\I_2}$=$P^{\I_1}$\\
%			\hspace*{0.2cm} for each atom $P(x_1,\ldots,x_k,y_1,\ldots,y_\ell)$ in $\psi(\vec{x},\vec{y})$~\footnote{WLOG we assume that all atoms with predicate $P$ in $\psi(\vec{x},\vec{y})$ have the form $P(x_1,\ldots,x_k,y_1,\ldots,y_\ell)$, where $x_1,\ldots,x_k$ belongs to $\vec{x}$ and $y_1,\ldots,y_\ell$ belongs to $\vec{y}$.}\\
%			\hspace*{0.6cm} $P^{\I_2}=P^{\I_2} \cup \{\tup{T_1,\ldots,T_k,U_1,\ldots,U_\ell}\}$\\[2mm]
%			%%
%			where, for $1 \leq i \leq k$, $T_i$ assumes one of the two following forms:
%			\begin{itemize}
%				\item $T_i=\mu(x_i)$, if $x_i$ is an entity-variable;
%				\item $T_i = \bigcap_{p=1}^{m}\mu(S_p^{x_i})$, if $x_i$ is value-variable and $\{S_1^{x_i},\ldots,S_m^{x_i}\}=\setvar(x_i,\trasf(\phi(\vec{x})))$;
%			\end{itemize} 
%			and for $1 \leq i \leq \ell$, $U_i=\{f_e^s\}$ if $y_i=y_e^s$, where $1 \leq s \leq h$, or $U_i=\{f_v^q\}$ if $y_i=y_v^q$, where $1 \leq q \leq j$.
%			%\begin{itemize}
%			%	\item $U_i=\{f_e\}$, where $f_e$ is an entity-null from $\Delta_{E_\bot}^{fresh}$ not occurring elsewhere in $P^{\I_2}$ and $\tup{T_1,\ldots,T_k,U_1,\ldots,U_\ell}$, if $y_i$ is an entity-variable;
%			%	\item $U_i=\{f_v\}$, where $f_v$ is a value-null from $\Delta_{V_\bot}^{fresh}$ not occurring elsewhere in $P^{\I_2}$ and $\tup{T_1,\ldots,T_k,U_1,\ldots,U_\ell}$, if $y_i$ is a value-variable. 
%			%\end{itemize} 						
%		\end{itemize}
%		%%
%		\item (entity-egd) let $d$ be an entity-egd of the form (\ref{eq:egd}). 
%		Let $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$ such that $\mu(y) \neq\mu(z)$. We say that $d$ is applicable to $\I_1$ with assignment $\mu$ (or analogously that $\mu$ triggers $d$ in $\I_1$), and we construct $\I_2=(\Delta^{\I_2},\sim^{\I_2}, \cdot^{\I_2})$ as follows:
%		\begin{itemize}
%			\item $\Delta^{\I_2}=\Delta^{\I_2}_E \cup \Delta^{\I_2}_V$, where $\Delta^{\I_2}_E=\Delta^{\I_1}_E$ and $\Delta^{\I_2}_V=\Delta^{\I_1}_V$
%			\item $\sim^{\I_2}=\sim^{\I_1} \cup \{\tup{f,g} \mid f,g \in \mu(y) \cup \mu(z)\}$;
%			\item $\cdot^{\I_2}$ is obtained from $\cdot^{\I_1}$ by replacing 
%			%each $[e]^{\sim{\I_1}}$  occurring the range of $\cdot^{\I_1}$, such that  $e \in \mu(x_1) \cup \mu(x_2)$, 
%			each occurrence of $\mu(y)$ and $\mu(z)$ 
%			%in the range of $\cdot^{\I_1}$ 
%			with $\mu(y) \cup \mu(z)$\nb{is this formal enough?}.
%			%			\item $e^{\I_2}=e^{\I_1}$, for each entity or entity-null $e \in \Delta_E^{\I_1}$ such that $e \not \in \mu(x_1) \cup \mu(x_2)$;
%			%			\item $v^{\I_2}=v^{\I_1}$, for each value or value-null $v \in \Delta_V^{\I_1}$;
%			%						\item $e^{\I_2}=\mu(x_1) \cup \mu(x_2)$, for each entity or entity-null $e \in \mu(x_1) \cup \mu(x_2)$;
%			%			\item $A^{\I_2}=\mathsf{repl}(A^{\I_1},\mu(x_1) \cup \mu(x_2))$, where the function $\mathsf{repl}(A^{\I_1},\mu(x_1) \cup \mu(x_2))$ replaces $\mu(x_1) \in A^{\I_1}$ and $\mu(x_2) \in A^{\I_1}$ (if any) with $\mu(x_1) \cup \mu(x_2)$, for each atomic concept $A$ in $\K$;
%			%			\item   $P^{\I_2}=\mathsf{repl}(P^{\I_1},\mu(x_1) \cup \mu(x_2))$, where the function $\mathsf{repl}(P^{\I_1},\mu(x_1) \cup \mu(x_2))$ replaces $\mu(x_1)$ and $\mu(x_2)$ occurring either as first or second component of a pair in $P^{\I_1}$ (if any) with $\mu(x_1) \cup \mu(x_2)$, for each atomic role $P$ in $\K$;
%			%			\item   $U^{\I_2}=\mathsf{repl}(U^{\I_1},\mu(x_1) \cup \mu(x_2))$, where the function $\mathsf{repl}(U^{\I_1},\mu(x_1) \cup \mu(x_2))$ replaces $\mu(x_1)$ and $\mu(x_2)$ occurring as first component of a pair in $U^{\I_1}$ (if any) with $\mu(x_1) \cup \mu(x_2)$, for each attribute $U$ in $\K$.
%		\end{itemize}
%		\item (value-egd) let $d$ be a value-egd of the form~(\ref{eq:egd}). Let $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$ such that $\mu(y) \neq\mu(z)$. 
%		%(i.e., $\mu(y)$ and $\mu(z)$ are different sets of values from $\Delta^{\I_1}_V$). 
%		We say that $d$ is applicable to $\I_1$ with assignment $\mu$ (or analogously that $\mu$ triggers $d$ in $\I_1$), and we construct $\I_2=(\Delta^{\I_2},\sim^{\I_2}), \cdot^{\I_2}$ as follows:
%		\begin{itemize}
%			\item $\Delta^{\I_2}=\Delta^{\I_2}_E \cup \Delta^{\I_2}_V$, where $\Delta^{\I_2}_E=\Delta^{\I_1}_E$ and $\Delta^{\I_2}_V=\Delta^{\I_1}_V$;
%			\item $\sim^{\I_2}=\sim^{\I_1}$;
%			\item $\cdot^{\I_2}$ is as  $\cdot^{\I_1}$ except for the interpretation of each predicate $P$ %such that there is an atom $P(t_1,\ldots,t_n)$ in $\phi(\vec{x})$ and an integer  $1\leq i \leq n$ for which it holds either $t_i=y$ or $t_i=z$. 
%			occurring in $\phi(\vec{x})$ in at least an atom having  $y$ and/or $z$ among its variables. For each such predicate we proceed as follows:
%			\begin{enumerate}
%				\item let $P(x_1,y,z,e_1,v_1),\ldots P(x_k,y,z,e_k,v_k)$ be the atoms in $\phi(\vec{x})$ having $P$ as predicate and $y$ and/or $z$ among their variables, where $x_i$ is an entity variable, $e_i$ is an entity, and $v_i$ is value, for each $1 \leq i \leq k$\footnote{WLOG we assume a fixed form for each such atom.}, and let $P(x_1,S_1^y,S_1^z,e_1,v_1),\ldots P(x_k,S_k^y,S_k^z,e_k,v_k)$ be the corresponding atoms in $\trasf(\phi(\vec{x}))$;
%				\item let $\IMG_{P_{\mu}}=P(\mu(x_1),\mu(S_1^y),\mu(S_1^z),\entitySet_1,\valueSet_1),\ldots,P(\mu(x_k),\mu(S_k^y),\mu(S_k^z),\entitySet_k,\valueSet_k)$ be the image of $P$ with respect to $\mu$;
%				\item $P^{\I_2}=P^{\I_1} \setminus \IMG_{P_{\mu}} \cup \NINT_P$, where $\NINT_P$  is obtained from $\IMG_{P_{\mu}}$ by replacing $\mu(S_i^y)$ and $\mu(S_i^z)$ with $\mu(S_1^y) \cup \ldots \cup \mu(S_k^y)\cup\ldots\cup \mu(S_1^z)\cup\ldots\cup\mu(S_k^z)$, for each $1\leq i \leq k$. 
%				%where $\{S_1^y,\ldots,S_n^y\}\subseteq\setvar(y,\trasf(\phi(\vec{x})))$, and $\{S_1^z,\ldots,S_m^z\}\subseteq\setvar(z,\trasf(\phi(\vec{x})))$
%			\end{enumerate}
%		\end{itemize}
%	\end{itemize}
%	Let $d$ be either a tgd or an entity-egd or a value-egd that can be applied to $\I_1$ with assignment $\mu$, we say that $\I_2$ is the result of applying $d$ to $\I_1$ with $\mu$ and we write $\I_1 \xrightarrow[]{d,\mu} \I_2$. We call $\I_1 \xrightarrow[]{d,\mu} \I_2$ a chase step. 
%\end{definition}

\begin{definition}[Chase Step] 
	\label{def:chaseStep}	
	Let $\K=(\T,\DB)$ be a KB, and let $\I_1$ be an instance for $\K$ \wrt an equivalence relation $\sim^1$ over $\underD_E(\I_1)$.
	
	%	and $\valuenulls$ and $\entitynulls$ be as defined above.
	\begin{itemize}
		\item (tgd) let $d$ be a tgd of the form (\ref{eq:tgd}). Without loss of generality we assume that all atoms in $\psi(\vec{x},\vec{y})$ have the form $P(x_1,\ldots,x_k,y_1,\ldots,y_\ell)$, where $x_1,\ldots,x_k$ belong to $\vec{x}$ and $y_1,\ldots,y_\ell$ belong to $\vec{y}$, and we denote with $\vec{y_e}=y_e^1,\ldots y_e^h$ and $\vec{y_v}=y_v^1,\ldots,y_v^j$ the entity-variables and value-variables in $\vec{y}$, respectively. Let $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$ such that there is no $\psi(\vec{x},\vec{y})$-compatible tgd-extension of  $\mu$ to $\I_1$.\nb{maybe we can assume that facts have the form $P(x,y)$ to slightly simplify the notation} 
		%%
		We say that $d$ is applicable to $\I_1$ with assignment $\mu$ (or analogously that $\mu$ triggers $d$ in $\I_1$),	and	construct $\I_2$ with the following procedure:\\[0.2cm]
            \hspace*{0.3cm} \textbf{let} $\{f_e^1,\ldots,f_e^h\} \subseteq \alphaEntityNulls$ and $\{f_v^1,\ldots,f_v^j\} \subseteq \alphaValueNulls$ be\\
            \hspace*{0.5cm}  two sets of fresh null symbols, i.e., not occurring in\\
            \hspace*{0.5cm}  $\I_1$, all distinct from each other\\
			\hspace*{0.3cm} $\I_2:=\I_1$\\
			\hspace*{0.3cm} \textbf{foreach} atom $P(x_1,\ldots,x_k,y_1,\ldots,y_\ell)$ in $\psi(\vec{x},\vec{y})$ \textbf{do}\\
			\hspace*{0.6cm} $\I_2:=\I_2 \cup \{P(T_1,\ldots,T_k,U_1,\ldots,U_\ell)\}$\\[2mm]
			%%
			where, 
			\begin{itemize}
				\item for $1 \leq i \leq k$, $T_i=\mu(x_i)$, if $x_i$ is an entity-variable, or $T_i = \bigcap_{p=1}^{m}\mu(S_p^{x_i})$, if $x_i$ is value-variable and $\{S_1^{x_i},\ldots,S_m^{x_i}\}=\setvar(x_i,\trasf(\phi(\vec{x})))$;
				\item for $1 \leq i \leq \ell$, $U_i=\{f_e^s\}$ if $y_i=y_e^s$, with $1 \leq s \leq h$, or $U_i=\{f_v^q\}$ if $y_i=y_v^q$, with $1 \leq q \leq j$.		
		  \end{itemize} 
	
			%where each $f_e^s$ (resp.\ $f_v^q$) is a fresh element from $\alphaEntityNulls$ ($\alphaValueNulls$)  not occurring elsewhere in $\I_2$.
		%%
		\item (entity-egd) let $d$ be an entity-egd of the form (\ref{eq:egd}). 
		Let $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$ such that $\mu(y) \neq\mu(z)$. We say that $d$ is applicable to $\I_1$ with assignment $\mu$ (or analogously that $\mu$ triggers $d$ in $\I_1$), and we construct $\I_2$ from $\I_1$ by replacing 
			in $\I_1$ each occurrence of $\mu(y)$ and of $\mu(z)$ with $\mu(y) \cup \mu(z)$.
		\item (value-egd) let $d$ be a value-egd of the form~(\ref{eq:egd}). Let $\mu$ be an assignment from $\phi(\vec{x})$ to $\I_1$ such that $\mu(y) \neq\mu(z)$, and let $\{S_1^y,\ldots,S_m^y\}=\setvar(y,\trasf(\phi(\vec{x})))$ and $\{S_1^z,\ldots,S_k^z\}=\setvar(z,\trasf(\phi(\vec{x})))$. We say that $d$ is applicable to $\I_1$ with assignment $\mu$ (or analogously that $\mu$ triggers $d$ in $\I_1$), and we construct %$\I_2=\I_1 \setminus \mu(\phi(\vec{x})) \cup \rho(\mu(\phi(\vec{x})) )$
		$\I_2$ from $\I_1$ by replacing in the image  $\mu(\phi(\vec{x}))$ (which is contained in $\I_1$) 
		each set $\mu(S_1^y),\ldots,\mu(S_m^y),\mu(S_1^z),\ldots$ and $\mu(S_k^z)$ with $\mu(S_1^y) \cup \ldots \cup \mu(S_m^y)\cup \mu(S_1^z)\cup\ldots\cup\mu(S_k^z)$.
	\end{itemize}
	Let $d$ be a tgd or entity-egd or value-egd that can be applied to $\I_1$ with assignment $\mu$, we say that $\I_2$ is the result of applying $d$ to $\I_1$ with $\mu$ and we write $\I_1 \xrightarrow[]{d,\mu} \I_2$. We call $\I_1 \xrightarrow[]{d,\mu} \I_2$ a chase step. \nb{Should we substitute $d$ with $r$?} 
\end{definition}

We refer the reader to the appendix for a comprehensive example of execution of the above chase steps over the KB we have used throughout the examples of this paper.\nb{In a final version we should put in the main body of the paper at least a portion of the example}

% \begin{example}
%     \label{ex:chase_step}
%     Consider the KB $\K=\tup{\T,\DB}$ in the Example~\ref{ex:query}. Let now $\I^\DB$ the \emph{base instance} composed by the following facts:

% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{llll}
% 			d1) & Emp([\textbf{\#Doe$_1$}], [\textbf{\#Yahoo}]) & d2) & CI([\textbf{\#Doe$_2$}], \{ \texttt{John Doe} \}, \{ \texttt{235-2635} \}) \\
% 			d3) & Emp([\textbf{\#Doe$_2$}], [\textbf{\#Yahoo}]) & d4) & CI([\textbf{\#Doe$_3$}], \{ \texttt{Mary Doe} \}, \{ \texttt{234-4358} \}) \\
% 			d5) & Emp([\textbf{\#Doe$_3$}], [\textbf{\#IBM}]) & d6) & CI(\textbf{[\#Doe$_4$}], \{ \texttt{J. Doe}\}, \{ \texttt{235-2635}\}) \\
% 			d7) & CI([\textbf{\#Doe$_1$}], \{ \texttt{J. Doe} \}, \{ \texttt{234-4358} \}) & d8) & CEO([\textbf{\#Doe$_1$}],[\textbf{\#Yahoo}]) \\
% 		\end{array}
% 	\end{align*}

% As an example of an applying a tgd $t$, let us apply the tgd $Emp(p,comp) \rightarrow CEO(comp,director) \wedge Pers(director)$ to $\I^{\DB}$. The tgd is applicable to $\I^{\DB}$ with the following assignment $\mu$:
% \[
% \begin{array}{lcl}
% 	\mu(p)&=&[\textbf{\#Doe$_1$}]\\
% 	\mu(comp)&=&[\mathbf{\textbf{\#Yahoo}}]\\
% \end{array}
% \]
% $\mu$ acts on fact $d1$. The chase step $\I^{\DB} \xrightarrow[]{t,\mu} \I_1$ produces $\I_1$ consisting by the following facts:

% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{llll}
% 			d1) & Emp([\textbf{\#Doe$_1$}], [\textbf{\#Yahoo}]) & d2) & CI([\textbf{\#Doe$_2$}], \{ \texttt{John Doe} \}, \{ \texttt{235-2635} \}) \\
% 			d3) & Emp([\textbf{\#Doe$_2$}], [\textbf{\#Yahoo}]) & d4) & CI([\textbf{\#Doe$_3$}], \{ \texttt{Mary Doe} \}, \{ \texttt{234-4358} \}) \\
% 			d5) & Emp([\textbf{\#Doe$_3$}], [\textbf{\#IBM}]) & d6) & CI(\textbf{[\#Doe$_4$}], \{ \texttt{J. Doe}\}, \{ \texttt{235-2635}\}) \\
% 			d7) & CI([\textbf{\#Doe$_1$}], \{ \texttt{J. Doe} \}, \{ \texttt{234-4358} \}) & d8)& CEO([\textbf{\#Doe$_1$}],[\textbf{\#Yahoo}]) \\
%             d9) & CEO([\textbf{\#$\bot_1$}],[\textbf{\#Yahoo}]) & d10) & Pers([\textbf{\#$\bot_1$}])
% 		\end{array}
% 	\end{align*}

% As an example of an applying an \emph{entity-egd} $e$, let us apply the formula $CEO(comp,director_1) \wedge CEO(comp,director_2) \rightarrow director_1 = director_2$ to $\I_1$. The egd is applicable to $\I_1$ with the following assignment $\mu$:
% \[
% \begin{array}{lcl}
% 	\mu'(comp)&=&[\mathbf{\textbf{\#Yahoo}}]\\
%     \mu'(director_1)&=&[\textbf{\#Doe$_1$}]\\
%     \mu'(director_2)&=&[\textbf{\#$\bot_1$}]\\
% \end{array}
% \]
% $\mu'$ acts on the facts $d8$ and $d9$. The chase step $\I_1 \xrightarrow[]{e,\mu'} \I_2$ produces $\I_2$ consisting by the following facts:
% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{llll}
% 			d1) & Emp([\textbf{\#Doe$_1$},\textbf{\#$\bot_1$}], [\textbf{\#Yahoo}]) & d2) & CI([\textbf{\#Doe$_2$}], \{ \texttt{John Doe} \}, \{ \texttt{235-2635} \}) \\
% 			d3) & Emp([\textbf{\#Doe$_2$}], [\textbf{\#Yahoo}]) & d4) & CI([\textbf{\#Doe$_3$}], \{ \texttt{Mary Doe} \}, \{ \texttt{234-4358} \}) \\
% 			d5) & Emp([\textbf{\#Doe$_3$}], [\textbf{\#IBM}]) & d6) & CI(\textbf{[\#Doe$_4$}], \{ \texttt{J. Doe}\}, \{ \texttt{235-2635}\}) \\
% 			d7) & CI([\textbf{\#Doe$_1$}], \{ \texttt{J. Doe} \}, \{ \texttt{234-4358} \})  \\
%             d9) & CEO([\textbf{\#Doe$_1$},\textbf{\#$\bot_1$}],[\textbf{\#Yahoo}]) & d10) & Pers([\textbf{\#Doe$_1$},\textbf{\#$\bot_1$}])
% 		\end{array}
% 	\end{align*}
% Note that we deleted $d8$ which is the same as $d9$ after propagating the replace of the newly discovered equivalence class over the new produced instance.

% As an example of an applying an \emph{value-egd} $v$, let us apply the formula $CI(p,name_1,phone_1)\wedge CI(p,name_2,phone_2) \rightarrow name_1=name_2$ to $\I_x$. Where $\I_x$ is obtained by applying serveral chase steps (all the steps can be found in the appendix). $\I_x$ consists of the following facts:
% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{llll}
% 			d1) & Emp([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}], [\textbf{\#Yahoo}]) & d2) & CI([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}], \{ \texttt{John Doe} \}, \{ \texttt{235-2635} \}) \\
% 			 &  & d4) & CI([\textbf{\#Doe$_3$}], \{ \texttt{Mary Doe} \}, \{ \texttt{234-4358} \}) \\
% 			d5) & Emp([\textbf{\#Doe$_3$}], [\textbf{\#IBM}]) & d6) & CI(\textbf{[\#Doe$_4$}], \{ \texttt{J. Doe}\}, \{ \texttt{235-2635}\}) \\
% 			d7) & CI([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}], \{ \texttt{J. Doe} \}, \{ \texttt{234-4358} \})  \\
%             d9) & CEO([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}],[\textbf{\#Yahoo}]) & d10) & Pers([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}])
% 		\end{array}
% 	\end{align*}

% The \emph{value-egd} is applicable to $\I_x$ with the following assignment $\mu$:
% \[
% \begin{array}{lcl}
% 	\mu''(p)&=&[\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}]\\
%     \mu''(name_1)&=&\{ \texttt{John Doe} \}\\
%     \mu''(name_2)&=&\{ \texttt{J. Doe} \}\\
%     \mu''(phone_1)&=&\{ \texttt{235-2635}\}\\
%     \mu''(phone_2)&=&\{ \texttt{234-4358} \}\\
% \end{array}
% \]
% $\mu''$ acts on the facts $d8$ and $d9$. The chase step $\I_x \xrightarrow[]{v,\mu''} \I_7$ produces $\I_7$ consisting by the following facts:
% 	\begin{align*}
% 		\arraycolsep=3.0pt
% 		\begin{array}{llll}
% 			d1) & Emp([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}], [\textbf{\#Yahoo}]) & d2) & CI([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}], \{ \texttt{John Doe}, \texttt{J. Doe} \}, \{ \texttt{235-2635} \}) \\
% 			 &  & d4) & CI([\textbf{\#Doe$_3$}], \{ \texttt{Mary Doe} \}, \{ \texttt{234-4358} \}) \\
% 			d5) & Emp([\textbf{\#Doe$_3$}], [\textbf{\#IBM}]) & d6) & CI(\textbf{[\#Doe$_4$}], \{ \texttt{J. Doe}\}, \{ \texttt{235-2635}\}) \\
% 			d7) & CI([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}], \{ \texttt{John Doe}, \texttt{J. Doe} \}, \{ \texttt{234-4358} \})  \\
%             d9) & CEO([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}],[\textbf{\#Yahoo}]) & d10) & Pers([\textbf{\#Doe$_1$},\textbf{\#Doe$_2$},\textbf{\#$\bot_1$}])
% 		\end{array}
% 	\end{align*}
% \qed
% \end{example}


%% OLD - uses intepretations
%%From the above definition it is easy to see that $\Delta^{\I_1} \subseteq \Delta^{\I_2}$, $\sim^{\I_1} \subseteq \sim^{\I_2}$, and thus that  $[e]^{\sim^{\I_1}} \subseteq [e]^{\sim^{\I_2}}$, for each entity $e \in \alphaEntities$. Furthermore, for each predicate $P$ and tuple $\tup{\genericSet_1,\ldots,\genericSet_n} \in P^{\I_1}$ there exists  $\tup{\genericSet_1',\ldots,\genericSet_n'} \in P^{\I_2}$  such that $T_i \subseteq T_i'$ for each $1 \leq i \leq n$. This last property follows from the fact that each chase step never deletes elements from the interpretation of predicates, and in an entity-egd step (resp.\ value-egd-step) it may substitute an equivalence class of entities (resp.\  a set of values) $T$ with a new set equivalence class (resp.\ set of values) containing $T$. \nb{this paragraph may be eliminated, since this property is formally, and more generally, stated in Proposition~\ref{pro:containment}}


%From the above definition it is easy to see that for each fact $P(\genericSet_1,\ldots,\genericSet_n) \in \I_1$ there exists  $P(\genericSet_1',\ldots,\genericSet_n') \in \I_2$  such that $T_i \subseteq T_i'$ for each $1 \leq i \leq n$. This last property follows from the fact that each chase step never deletes elements from the interpretation of predicates, and in an entity-egd step (resp.\ value-egd-step) it may substitute an equivalence class of entities (resp.\  a set of values) $T$ with a new set of entities (resp.\ set of values) containing $T$. \nb{this paragraph may be eliminated, since this property is formally, and more generally, stated in Proposition~\ref{pro:containment}}

We next prove that $\I_2$ produced by a chase step from an instance $\I_1$ for $\K$ is in turn an instance for $\K$.

\begin{proposition}
	\label{prop:chase-interpretation}
	Let $\K$ be a KB, let $\I_1$ be an instance for $\K$ \wrt an equivalence relation $\sim^1$ over $\underD_E(\I_1)$, and let $\I_2$ be such that $\I_1 \xrightarrow[]{d,\mu} \I_2$. Then, there is an equivalence relation $\sim^2$ over a set $\S_2$ such that $\I_2$ is an instance for $\K$ \wrt $\sim^2$ over $\underD_E(\I_2)$.\nb{unclear if over $\underD_E(\I_2)$ is really needed. } Moreover, $\sim^1 \subseteq \sim^2$ and $\underD(\I_1) \subseteq \underD(\I_2)$.\nb{Check whether these last two properties are really needed (in particular, the last one)}
\end{proposition}

\begin{proof}
	We prove the thesis by considering the three possible cases for the rule $d$ and the corresponding chase steps of Definition~\ref{def:chaseStep}.
	
	\emph{Case of tgd chase step:} Let $d$ be a tgd of the form (\ref{eq:tgd}). In this case $\S=\underD_E(\I_1) \cup \textsf{N}^{f_e}$, where $\textsf{N}^{f_e}=\{f_e^1,\ldots,f_e^h\} \subseteq \alphaEntityNulls$ and $\sim^2=\sim^1 \cup \{\tup{f,f}~|~f \in \textsf{N}^{f_e}\}$	(notice that $\textsf{N}^{f_e}$ 
		could even be empty, which implies $\sim^2=\sim^1$). It is easy to see that $\sim^2$ is an equivalence relation over $\S$,  and that $\underD_E(\I_1)/{\sim^1} \subseteq \S/{\sim^2}$, and thus for each $P(\genericSet_1,\ldots,\genericSet_n) \in \I_2$  and each $1 \leq i \leq n$ such that $\type(P,i)=\entity$, either $T_i \in \underD_E(\I_1)/{\sim^1}$, and thus  $\genericSet_i \in  \S/{\sim^2}$, or $\genericSet_i =\{f\}$, where $f \in \textsf{N}^{f_e}$, and from the definition of $\sim^2$ it obviously holds that $\{f\} \in  \S/{\sim^2}$. Notice also that $\S=\underD_E(\I_2)$.  Moreover, for each $1 \leq i \leq n$ such that $\type(P,i)=\val$, it holds either $T_i \subseteq \underD_V(\I_1)$ or $T_i=\{f'\}$, where $f' \in \{f_v^1,\ldots,f_v^j\} \subseteq \alphaValueNulls$. Thus, $T_i$ is a non-empty subset of $(\alphaValues \cap \sig(\K))\cup \alphaValueNulls$. The above facts show that $\I_2$ is an instance for $\K$ \wrt $\sim^2$ over $\S=\underD(\I_2)$. 
		By construction, we also have $\sim^1 \subseteq \sim^2$. Moreover, $\underD_V(\I_2)=\underD_V(\I_1) \cup \{f_v^1,\ldots,f_v^j\}$ and thus $\underD(\I_1) \subseteq \underD(\I_2)$\nb{The last two sentences should be dropped if we do not want to give these results in the theorem}
		
	\emph{Case of entity-egd chase step:} 
%%
Let $d$ be an entity-egd of the form (\ref{eq:egd}).  In this case $\S=\underD_E(\I_1)$ and $\sim^2=\sim^1 \cup \sim^e$, where $\sim^e = \{\tup{f,g} \mid f,g \in \mu(y) \cup \mu(z)\}$. Obviously, $\sim^{e}$ is an equivalence relation over $\mu(y) \cup \mu(z)$. Thus $\sim^2$ is the union of an equivalence relation over $\underD_E(\I_1)$ and an equivalence relation over $\mu(y) \cup \mu(z)$. 
%%
As a consequence, $\sim^2$ is a reflexive and symmetric  relation over $ \underD_E(\I_1) \cup \mu(y) \cup \mu(z)$, and since $\mu(y) \cup \mu(z) \subseteq \underD_E(\I_1)$, then $\sim^2$ is reflexive and symmetric  over $\S$. We have then to prove that  $\sim^2$ is also transitive over $\S$. To this aim we consider all possible cases. Let $a,b,c$ be elements in $\S$. The following situations are conceivable:
	\begin{itemize}
		\item $(a,b) \in \sim^1$ and $(b,c) \in \sim^1$, but since $\sim^1$ is an equivalence relation over $\underD_E(\I_1)=\S$,  then  $(a,c) \in \sim^1$, and since $\sim^1 \subseteq \sim^2$ then $(a,c) \in \sim^2$.
		\item $(a,b) \in \sim^{e}$ and $(b,c) \in \sim^{e}$, but since $\sim^{e}$ is an equivalence relation over $\mu(y) \cup \mu(z)$, then $(a,c) \in \sim^{e}$ and since $ \sim^{e}\subseteq \sim^2$ then $(a,c) \in \sim^2$.
		\item $(a,b) \in \sim^1$ and $(b,c) \in \sim^{e}$.  Since  $(b,c) \in \sim^{e}$, by definition of chase step, $b,c \in \mu(y) \cup \mu(z)$, and also $[b]_{\sim^1}\subseteq \mu(y) \cup \mu(z)$. Since  $(a,b) \in \sim^1$, it also holds that  $a \in [b]^{\sim^{\I_{1}}}$, and thus  $a\in \mu(y) \cup \mu(z)$. This means that $(a,b) \in \sim^{e}$ as well, which coincides with the previous case (for which we have already shown that transitivity holds).
	\end{itemize}
	%%	
	We can then prove that each fact $P(T_1,\ldots,T_n)$ of $\I_2$ satisfies the conditions of Definition~\ref{def:instance} with an argument similar to that used in the last part of the proof for the tgd case. The only difference is that if some $T_i$ does not occur also in some fact of $\I_1$, then it must be $T_i=\mu(z) \cup \mu(y)$,  %(whereas in the tgd case $T_i=\{f\}$, where $f$ is a fresh null), 
	which is indeed an equivalence class of $\S/\sim^2$. Moreover, it obviously holds that $\sim^1 \subseteq \sim^2$ and $\underD(\I_2) = \underD(\I_1)$.\nb{The last sentence should be dropped if we do not want to give these results in the theorem}
	
	\emph{Case of value-egd chase step:} 
%%
Let $d$ be a value-egd of the form (\ref{eq:egd}). In this case $\S=\underD_E(\I_1)$ and $\sim^2=\sim^1$. So, in this case we do not have to construct a new equivalence relation. 
	%%
	The rest of the proof proceeds as for the previous cases. We however note that in this case each $T_i$ that does not occur in a fact of $\I_1$ must be of the form $\mu(S_1^y) \cup \ldots \cup \mu(S_m^y)\cup \mu(S_1^z)\cup\ldots\cup\mu(S_k^z)$, which is clearly a non-empty subset of $(\alphaValues \cap \sig(\K))\cup \alphaValueNulls$. We conclude the proof by remarking that $\sim^1 = \sim^2$ and obviously $\underD(\I_2) = \underD(\I_1)$.\nb{The last sentence should be dropped if we do not want to give these results in the theorem}
\end{proof}


%Let $d$ be either an inclusion assertion or an entity resolution rule, we define $head(d)$ the conjunction of the atom in right hand side of $d$ and with $body(d)$ the left hand side.

A chain of chase steps constitutes a chase sequence, as formally defined below.

\begin{definition}[Chase sequence]
	\label{def:chaseSequence}
	Let $\K=\tup{\T,\DB}$ be a KB, a \emph{chase sequence for $\K$} is a sequence (finite or infinite) $\I_0,\I_1, \I_2\dots$, such that $\I_0=\I^\DB$, $\I_i \xrightarrow[]{d_i,\mu_i} \I_{i+1}$ is a chase step,  %where $d_i$ is a tgds in $\T$ or an entity resolution rule in $\E$, and $\mu_i$ is an assignment that triggers $d_i$ in $\I_i$, 
	for each pair $\I_i,\I_{i+1}$ in the sequence. 
\end{definition}

%\begin{example}
%    Considering the Example~\ref{ex:chase_step} a chase sequence is $\I^\DB,\I_1,\I_2$.
%\end{example}

%By Proposition~\ref{prop:chase-interpretation} and the fact that $\I^\DB$ is an instance for $\K$ it follows that all the elements in a chase sequence for $\K$ are instances for $\K$. 
We define the length of a chase sequence $\sigma$, denoted $\len(\sigma)$, as the number of instances occurring in $\sigma$. When the sequence $\sigma$ is infinite, we write $\len(\sigma)=\infty$. \nb{check whether $\len$ is really used}

The following proposition easily follows from Proposition~\ref{prop:chase-interpretation} and the fact that in every chase sequence $\I_0=\I^\DB$ and  $\I^\DB$ is an instance for $\K$ by construction. 

\begin{proposition}
	\label{pro:chase-step-interpretation}
	Every $\I_i$ occurring in a chase sequence $\sigma$ for a KB $\K=\tup{\T,\DB}$ is an instance for $\K$.   
\end{proposition}




We next provide some useful properties holding for pairs of instances in a chase sequence .

\begin{proposition}
	\label{pro:containment}
	Let $\K=\tup{\T,\DB}$ be a KB, $\sigma$ be a chase sequence for $\K$, $\I_i$ and $\I_j$ be two instances for $\K$ \wrt equivalence relations $\sim^i$ and $\sim^j$, respectively, such that $\I_i$ and $\I_j$  belong to $\sigma$ and $i \leq j$, and let $P(\vec{\genericSet}$ be a fact in  ${\I_i}$. Then, it holds that $(i)$ $\sim^i \subseteq \sim^j$, $(ii)$ $\underD(\I_i) \subseteq \underD(\I_j)$, and
	%and  $[e]^{\sim^{\I_i}} \subseteq [e]^{\sim^{\I_j}}$, for each entity $e \in \alphaEntities$.
	$(iii)$ there exists  $P(\vec{\genericSet'}) \in \I_j$  such that $P(\vec{\genericSet}) \leq P(\vec{\genericSet}')$.
%$T_k \subseteq T_k'$ for each $1 \leq k \leq n$.
\end{proposition}

\begin{proof}
	The properties can be easily proved by induction.
	%%
	\emph{Base case.} Let be $i=0$ and $j=1$, that is, consider $\I_0$ and $\I_1$, where $\I_0$ is the base instance $\I^\DB$ of $\DB$ and $\I_1$ is the instance produced by the application of a chase step to $\I^\DB$. The inclusions $\sim^0 \subseteq \sim^1$ and $\underD(\I_0) \subseteq \underD(\I_1)$can be proved as in Proposition~\ref{prop:chase-interpretation}.	It remains to prove that for each fact $P(\vec{\genericSet}) \in \I_0$ there exists  $P(\vec{\genericSet'}) \in \I_1$  such that $\vec{\genericSet} \leq \vec{\genericSet'}$. Let us consider the three possible chase steps. \emph{(tgd)}: this step does not modify facts in $\I_0$, thus $\vec{\genericSet}=\vec{\genericSet'}$. \emph{(entity-egd)}: every equivalence class $E$ in $\activeD(\I_0)$, i.e., the active domain of $\I_0$, remains as is or it is substituted by a class $E'$ such that $E\subseteq E'$. Moreover, $\activeD_V(\I_0)=\activeD_V(\I_1)$. These facts easily show the thesis in this case. \emph{(value-egd)}: the argument is similar as the previous case, that is, every set of values $\valueSet$ in $\activeD_V(\I_0)$ remains as is or it is substituted by a set of values $\valueSet'$ such that $\valueSet\subseteq \valueSet'$. Moreover, $\activeD_E(\I_0)=\activeD_E(\I_1)$. 
	
	%%
	\emph{Inductive case.} we assume that the thesis holds for a certain integer $\ell$, i.e., that properties $(i)$, $(ii)$, and $(iii)$ hold for each $i,j \leq \ell$ such that $i \leq j$, and prove that they hold also for each $i,j \leq \ell+1$ such that $i \leq j$. The only cases that need to be shown are those in which $j=\ell+1$, because the other cases already hold by the inductive hypothesis.
	%%
	Of course, if $i =\ell+1$ the condition is trivially satisfied. For $i=\ell$ the three properties can be proved exactly as done for the base case. Then, all cases in which $i<\ell$ follow by the previous case and the inductive hypothesis.
\end{proof}

We notice also that from property $(i)$ of Proposition~\ref{pro:containment}, it follows that for every $i\leq j$ and every equivalence class $E \in \underD_E(\I_i) /{\sim^i}$ there exists $E' \in \underD_E(\I_j) /\sim^j$ such that $E \subseteq E'$, and in particular $[e]_{\sim^i} \subseteq [e]_{\sim^j}$, for each entity $e \in \alphaEntities \cap \sig(\K)$.


As for the standard chase~\cite{CDLLR07}, when the chase sequence for a KB is infinite there might be rules applicable to a certain instance $\I_i$ in the sequence that are never applied, though they remain applicable in next chase steps.\nb{The assignment might change, because equivalence classes and sets of values of the original assignment might be substituted by subsets thereof, but hopefully we do not need to enter in these details.} It is however always possible to establish a suitable order in the application of the rules so that the above phenomenon never occurs. Chase sequences enjoying this property are called \emph{fair}. In the following we assume that all chase sequences we consider are fair. 
%%%and we simply call one such sequence  \emph{the chase sequence for a KB $\K$}, and denote it with $\chaseSeq(\K)$.\nb{check whether something similar is really needed in the following. I am however not sure it is correct to refer to only one sequence. This seems appropriate only if the result of the chase is always a universal solution (which for the infinite case we are not able to prove).}


We now provide the definition of the result of the chase for a KB $\K$. We first deal with the case in which the chase procedure terminates and then consider the case in which it is constituted by infinitely many steps.

\subsection{Terminating chase procedure}

We first provide the definition of the result of the chase for finite chase sequences.

%We consider a KB $\K$ such that $\chaseSeq(\K)$ is finite, i.e., $\len(\chaseSeq(\K))=m$ where $m$ is an integer. 
%%
%\begin{definition}
%\label{def:chase-finite-case}
%    Let $\K$ be a KB such that $chaseSeq(\K)=\I_0,\I_1,\ldots,\I_m$ where $m \in \mathbb{N}$. Then, we call \emph{$\I_k$ the chase of $\K$} and denote it with $\chase(\K)$.
%\end{definition}

\begin{definition}[Finite Chase]
	\label{def:chase-finite-case}
	Let $\K=\tup{\T,\DB}$ be a KB. A \emph{finite chase of $\K$} is a finite chase sequence $\I_0,\I_1,\ldots,\I_m$, %where $m \in \mathbb{N}$. 
	such that there is no rule $r$ in $\T$ and no assignment $\mu$ such that $r$ can be applied to $\I_m$ with $\mu$. We say that $\I_m$ is the \emph{result of the finite chase for $\K$}, and denote it with $\chase(\K)$.
\end{definition}

From Proposition~\ref{pro:chase-step-interpretation} it follows that $\chase(\K)$ is an instance for $\K$. Below we show that it is indeed also a solution.

\begin{lemma}
	\label{lem:chase-finite-case-model}
	Let $\K$ be a KB and let $\I_0,\I_1,\ldots,\I_m$ be a finite chase for $\K$. Then $\chase(\K)$ is a solution for $\K$.
\end{lemma}

\begin{proof}
	We need to prove that $\chase(\K)$ satisfies all facts in $\DB$, all tgds, entity-egds and value-egds in $\T$. We show each point separately:
	\begin{itemize}%\itemsep-1em 
		\item[(i)] The property that $chase(\K)$ satisfies all facts in $\DB$ follows from $\I_0=\I^\DB$ and from Proposition~\ref{pro:containment}. Indeed, $\I^\DB$ satisfies all facts in $\DB$, by definition of base instance, which means that for each ground atom $P(c_1,\ldots,c_n)$ in $\DB$ there is a fact $P(\genericSet_1,\ldots,\genericSet_n)$ in $\I_0$ such that $c_i \in T_i$ for $1 \leq i\leq n$. By Proposition~\ref{pro:containment} it follows that in $\I_m$ there is a tuple $\tup{T_1',\ldots,T_n'}$ such that $T_1 \subseteq T_1',\ldots,T_n \subseteq T_n'$, and thus $P(c_1,\ldots,c_n)$ is satisfied also in $\I_m=chase(\K)$.
		\item[(ii)] To prove that $chase(\K)$ satisfies all tgds in $\T$, let us assume by contradiction that there is a tgd $d = \forall \vec{x}(\phi(\vec{x}) \rightarrow \exists \vec{y} \psi(\vec{x}, \vec{y}))$ that is not satisfied by $chase(\K)$. This means that there is an assignment $\mu$ from $\phi(\vec{x})$ to $\chase(\K)$ such that there is no $\psi(\vec{x},\vec{y})$-compatible tgd-extension $\mu'$ of $\mu$ to $\chase(\K)$. But thus $d$ would be applicable to $\chase(\K)$ with assignment $\mu$, which contradicts the hypothesis that $\sigma$ is a finite chase.
		%is triggered by $\mu$ in an interpretation $\I_i$ belonging to $\chaseSeq(\K)$, and from Proposition~\ref{pro:will-be-triggered} we get a contradiction.
		\item[(iii)] The fact that $chase(\K)$ satisfies all the entity-egds and value-egds can be proved as done in (ii) for satisfaction of tgds in $\T$.
	\end{itemize}
\end{proof}

%% Triangle Lemma

The following Lemma will be exploited to prove that $\chase(\K)$ is not simply a solution for $\K$, but it is also universal. A similar Lemma has been used in~\cite{FKMP05} to prove an analogous result in the context of Data Exchange.


%In the proof of the Lemma, we use the following notation:  if $\I$ is an interpretation, $P$ is an $n$-ary predicate, and $\tup{T_1,\ldots,T_n} \in P^{\I}$, we say that the $P(T_1,\ldots,T_n)$ is a $P$-fact in $\I$, or simply facts when $P$ is clear from the context (remember also that $\tup{T_1,\ldots,T_n}$ is a tuple of equivalence classes in $\Delta^\I/{\sim^\I}$ and sets of values in $\powersetnoempty(\Delta^\I_V)$). Then, ${\rm Facts}(\I)$ denotes the set of the facts of $\I$, while $|{\rm Facts}(I)|$ denotes the cardinality of the set of the facts of $I$.\nb{This notation is introduced again in the next section. We should however anticipate it somewhere in the framework. BTW we should say that this is an ``interpretation fact'', not to be confused with a ``standard'' fact (which is syntactic and belongs to the database).}


\begin{lemma}
	\label{lem:triangle-finite-case}
	%Let $\K=\tup{\T,\DB,\E}$ be a $\KER$, and 
	Let $\I_{1} \xrightarrow[]{d,\mu} \I_{2}$ be a chase step.
	%in the chase sequence for $\K$. 
	Let $\I$ be an instance for $\K$ such that: ($i$) $\I$ satisfies $d$ and ($ii$) there exists a homomorphism $h_1: \I_1\rightarrow \I$. Then there exists a homomorphism $h_2: \I_2\rightarrow \I$. Furthermore, $h_2$ extends $h_1$.\nb{the extension property is not needed (we hilighted it because of our attempts to define the result of the chase for the infinite case). However, the proof is for free, and we can maintain it.}
\end{lemma}

\begin{proof}
	
	The proof follows the line of the proof of Lemma 3.4 in \cite{FKMP05}. However, since our structures are based on equivalence classes and sets of values, the various steps of the proof are more involved. In particular, differently from~\cite{FKMP05}, in our framework the composition of an assignment with an homomorphism does not directly yield a new assignment. However, an assignment can be constructed on the basis of such composition.
	
	We prove the thesis by considering the three possible cases for the rule $d$ and the corresponding chase steps of Definition~\ref{def:chaseStep}.
	
	\emph{Case of tgd chase step:} Let $d$ be a tgd of the form (\ref{eq:tgd}). For ease of exposition, we  assume $\phi(\vec{x}) = P_1(x_1,x_2) \land P_2(x_1,x_2)$ and $\psi(\vec{x},\vec{y})=P_3(x_1,x_2,y_1,y_2) \land P_4(x_2,y_1,y_2)$, where $x_1$ and $y_2$ are entity variables and $x_2$ and $y_1$ are value-variables\nb{this tgd contains all interesting possible cases:  join of entity- and value-variables in the body, the same variables are propagated to the head of the tgd, where both existential entity- and value-variable exist, both forming a join.}. The case of generic tgds can be managed in a similar way.
	%%
	If we apply the operator $\tau$ to both the body and the head of the tgd, we obtain the following formulas:\\
	$\tau(\phi(\vec{x}))=P_1(x_1,S_1^{x_2})\land P_2(x_1,S_2^{x_2})$\\
	$\tau(\psi(\vec{x},\vec{y}))=P_3(x_1,R_1^{x_2},R_1^{y_1},y_2)\land P_4(R_2^{x_2},R_2^{y_1},y_2)$\\
	%%
	We first construct an assignment $\hat{\mu}$ from $\phi(\vec{x})$ to $\I$.   By the definition of chase step, $\mu$ is an assignment from $\phi(\vec{x})$ to $\I_1$. Then, there exist an equivalence class $E_1 \in \activeD_E(\I_1)$ and two sets of values $V_1,V_2 \in \activeD_V(\I_1)$ such that $V_1 \cap V_2 \neq \emptyset$, $\mu(x_1)=E_1$, $\mu(S_1^{x_2})=V_1$, $\mu(S_2^{x_2})=V_2$, $P_1(E_1,V_1)$ and $P_2(E_1,V_2)$ are facts in $\I_1$.
	%%
	Since $h_1$ is homomorphism from $\I_1$ to $\I$, there exist facts $P_1(E_1',V_1')$, $P_2(E_2',V_2')$ in $\I$, 
	%%where $E_1',E_2' \in \Delta^\I/{\sim^\I}$ and $V_1',V_2' \in \powersetnoempty(\Delta_V^\I)$,
	such that $h_1(E_1)\subseteq E_1'$, $h_1(E_1)\subseteq E_2'$, $h_1(V_1)\subseteq V_1'$, $h_1(V_2)\subseteq V_2'$. 
	Since $V_1 \cap V_2 \neq \emptyset$, then also $V_1' \cap V2' \neq \emptyset$. Moreover, since $E_1'$ and $E_2'$ are equivalence classes containing the same non-empty subset, they must be the same equivalence class, i.e., $E_1'=E_2'$. We then define the mapping $\hat{\mu}$  as follows: $\hat{\mu}(x_1)=E_1'$, $\hat{\mu}(S_1^{x_2})=V_1'$, and $\hat{\mu}(S_2^{x_2})=V_2'$. It is easy to see that $\hat{\mu}$ satisfies the conditions in Definition~\ref{def:assignment-revisited}, and thus it  is an assignment from $\phi(\vec{x})$ to $\I$.
	
	Since $\I$ satisfies $d$, there is an assignment $\mu'$ that is a $\psi(\vec{x},\vec{y})$-compatible extension of $\hat{\mu}$ to $\I$. By definition we have that: 
	\begin{itemize}
		\item $\mu'(x_1)=\hat{\mu}(x_1)=E_1'$
		\item $\mu'(R_1^{x_2})=V_3'$, $\mu'(R_2^{x_2})=V_4'$, where $V_3',V_4' \in \activeD_V(\I)$ are such that $V_1' \cap V_2' \subseteq V_3' \cap V_4'$,
		\item $\mu'(R_1^{y_1})=V_5'$, $\mu'(R_2^{y_1})=V_6'$, where $V_5',V_6' \in \activeD_V(\I)$ are such that $V_5' \cap V_6' \neq \emptyset$,
		\item $\mu'(y_2)=E_2'$, where $E_2' \in \activeD_E(\I)$,
		\item $\I$ contains the facts $P_3(E_1',V_3',V_5',E_2')$ and $P_4(V_4',V_6',E_2')$.
	\end{itemize}
	
	%%
	Then, by definition of tgd chase step it follows that there is also an assignment $\mu_2$ from $\psi(\vec{x},\vec{y})$ to $\I_2$ defined as follows
	\begin{itemize}
		\item $\mu_2(x_1)=\mu(x_1)=E_1$
		\item $\mu_2(R_1^{x_2})=\mu_2(R_2^{x_2})=V_1 \cap V_2$
		\item $\mu_2(R_1^{y_1})=\mu_2(R_2^{y_1})=\{f_v^{y_1}\}$
		\item $\mu_2(y_2)=[f_e^{y_2}]$
	\end{itemize}
	where $f_v^{y_1}$ and $f_e^{y_2}$ are the fresh value-null and entity-null, respectively, introduced by the chase step. We remark that $\mu_2$ is a $\psi(\vec{x},\vec{y})$-compatible extension of $\mu$ to $\I_2$, and that $\underD(\I_2)=\underD(\I_1) \cup \{f_v^{y_1},f_e^{y_2}\}$. Moreover, $\I_2= \I_1 \cup \{P_3(E_1,V_1 \cap V_2, \{f_v^{y_1}\},[f_e^{y_2}]),P_4(V_1 \cap V_2, \{f_v^{y_1}\},[f_e^{y_2}])\}$.
	%%
	
	We now construct a mapping $h_2$ %from the elements of $\underD(\I_2)$ to the elements of $\underD(\I)$ 
	and show that it is an homomorphism from $\I_2$ to $\I$.
	%%
	We define $h_2$ as follows:
	\begin{itemize}
		\item $h_2(o)=h_1(o)$ for each $o \in \underD(\I_1)$;
		\item $h_2(f_v^{y_1})=v$, where $v$ is any element in $V_5' \cap V_6'$;
		\item $h_2(f_e^{y_2})=e$, where $e$ is any element in $E_2'$.
	\end{itemize}
	Note that, as stated before, $V_5' \cap V_6' \neq \emptyset$. Moreover, $E_2' \neq \emptyset$, since $E_2'$ is an equivalence class in $\activeD(\I)$. Thus $v$ and $e$ above always exist. %$h_2(f_v^{y_1})$  and $h_2(f_e^{y_2})$ are well defined.
	Note also that $h_2$ extends $h_1$.
	
	By construction, $h_2$ is a mapping from the elements of $\underD(\I_2)$ to the elements of $\underD(\I)$. Moreover, Conditions~1-4 of Definition~\ref{def:homomorphism} (homomorphism) are trivially satisfied.
	To prove that $h_2$ is homomorphism from $\I_2$ to $\I_1$ it remains to prove that also Condition~5 of Definition~\ref{def:homomorphism} holds. 
	%%
	Such condition is obviously satisfied by all facts in $\I_1$, since $h_2$ over such facts behaves as $h_1$, and $h_1$ is an homomorphism to $\I$. 
	%%
	Consider now the fact $P_3(E_1,V_1 \cap V_2, \{f_v^{y_1}\},[f_e^{y_2}])$, which is in $\I_2\setminus \I_1$. We have to show that there exists a fact in $\I$ of the form $P_3(\hat{E_1},\hat{V_1},\hat{V_2},\hat{E_2})$, where $\hat{E_1},\hat{E_2} \in \activeD_E(\I)$ and $\hat{V_1},\hat{V_2} \in \activeD_V(\I)$, 
	such that $h_2(E_1) \subseteq\hat{E_1}$, $h_2(V_1 \cap V_2)\subseteq \hat{V_1}$, $h_2( \{f_v^{y_1}\})\subseteq \hat{V_2}$,  $h_2( [f_e^{y_2}])\subseteq \hat{E_2}$.
	%%
	To this aim we set $\hat{E_1}=E_1'$, $\hat{V_1}=V_3'$, $\hat{V_2}=V_5'$, $\hat{E_2}=E_2'$, and show that the above mentioned containments do indeed hold.
	\begin{itemize}
		\item $h_2(E_1) \subseteq E_1'$ follows from $h_2(E_1)=h_1(E_1)$ and $h_1(E_1) \subseteq E_1'$;
		\item $h_2(V_1 \cap V_2) \subseteq V_3'$ is a consequence of $h_2(V_1 \cap V_2)=h_1(V_1 \cap V_2) \subseteq h_1(V_1) \cap h_1(V_2) \subseteq V_1' \cap V_2' \subseteq V_3' \cap V_4' \subseteq V_3'$. 
		%%In particular, to show that $h_1(V_1 \cap V_2) \subseteq h_1(V_1) \cap h_1(V_2) $, consider any $b \in h_1(V_1 \cap V_2)$, i.e., $b=h_1(v)$ with $v \in V_1 \cap V_2$. Obviously, this means that $b \in h_1(V_1)$ and $b \in h_1(V_2)$, and thus $b \in h_1(V_1) \cap h_1(V_2)$. To show that $h_1(V_1) \cap h_1(V_2) \subseteq V_1' \cap V_2'$ it is sufficient to recall that $h_1(V_1) \subseteq V_1'$ and $h_1(V_1) \subseteq V_2'$. 
		\item $h_2(\{f_v^{y_1}\}) \subseteq V_5'$ holds because $h_2(f_v^{y_1})=v$ and $v \in V_5' \cap V_6'$, and thus $h_2(\{f_v^{y_1}\})=\{v\} \subseteq V_5'$.
		\item $h_2([f_e^{y_2}]) \subseteq E_2'$ holds because $h_2(f_v^{y_1})=e$ and $e \in E_2'$, and thus $h_2([f_e^{y_2}])=[e] \subseteq E_2'$.
	\end{itemize}
	We can proceed in analogously to show that Condition~5 of Definition~\ref{def:homomorphism} is satisfied also for the other fact, $P_4(V_1 \cap V_2, \{f_v^{y_1}\},[f_e^{y_2}])$, which is contained in $\I_2 \setminus \I_1$.
	
	\emph{Case of entity-egd chase step:} 
	%%
	Let $d$ be an entity-egd of the form (\ref{eq:egd}). 
	%%
	By the definition of the chase step, $\mu$ is an assignment from $\phi(\vec{x})$ to $\I_1$, and in particular there exist equivalence classes $E_1,E_2 \in \activeD_E(\I_1)$ such that $\mu(y)=E_1$ and  $\mu(z)=E_2$.
	%%
	It is then possible to construct an assignment $\hat{\mu}$ from $\phi(\vec{x})$ to $\I$ such that $\hat{\mu}(y)=E_1'$, $\hat{\mu}(z)=E_2'$, $E_1',E_2' \in \activeD_E(\I_1)$, $h_1(E_1) \subseteq E_1'$ and $h_1(E_2) \subseteq E_2'$.
	%%
	The construction of $\hat{\mu}$ is similar to the analogous construction described for the case of tgd chase step. For the sake of completeness we describe this procedure also for the entity-egd chase step (note that in this case we need to also deal with entities and values possibly occurring in the rule body $\phi(\vec{x})$). For ease of exposition, and without loss of generality, we assume that $\phi(\vec{x})=P_1(x,y,e,v) \land P_2(x,y,z)$, where $x$ is a value-variable, $y,z$ are entity-variables, $e \in \alphaEntities$, and $v \in \alphaValues$. By applying the operator $\tau$ to $\phi(\vec{x})$ we obtain
	$\tau(\phi(\vec{x}))=P_1(S_1^{x},y,e,v)\land P_2(S_2^{x},y,z)$. Since $\mu$ is an assignment from $\phi(\vec{x})$ to $\I_1$, there exists $E,E_1,E_2 \in \activeD_E(\I_1)$  and $V,V_1,V_2 \in \activeD_V(\I_1)$ such that $e \in E$, $V_1 \cap V_2 \neq \emptyset$, $v \in V$, $P_1(V_1,E_1,E,V)$ and $P_2(V_2,E_1,E_2)$ are two facts in $\I_1$, and $\mu(S_1^x)=V_1$, $\mu(y)=E_1$, $\mu(v)=V$, $\mu(S_2^x)=V_2$, and $\mu(z)=E_2$.
	%%
	Since $h_1$ is homomorphism from $\I_1$ to $\I$, there exist $E',E_1',E_2' \in \activeD_E(\I)$ and $V',V_1',V_2' \in  \activeD_V(\I)$ such that $h_1(E_1) \subseteq E_1'$, $h_1(V_1) \subseteq V_1'$, $h_1(E) \subseteq E'$, $h_1(V) \subseteq V'$, $h_1(V_2) \subseteq V_2'$, $h_1(E_2) \subseteq E_2'$ and $P_1(V_1',E_1',E',V')$ and $P_2(V_2',E_1',E_2')$ are two facts in $\I$. We then define $\hat{\mu}$ as follows: $\hat{\mu}(S_1^x)=V_1'$, $\hat{\mu}(y)=E_1'$, $\hat{\mu}(v)=V$, $\hat{\mu}(S_2^x)=V_2'$, $\hat{\mu}(z)=E_2'$.
	%%
	It is easy to see that $\hat{\mu}$ is an assignment from $\phi(\vec{x})$ to $\I$. In particular, since $e \in E$ and $h(e)=e$ it obviously holds $e \in h_1(E) \subseteq E'$, which implies  $e \in E'$. Similarly, since $v \in \mu(v)=V$ and $v=h_1(v)$ we have that $v \in h_1(V) \subseteq V'$, which implies  $v \in V'$.

	
	We then take $h_2$ to be $h_1$ and show that $h_1$ is still a homomorphism when considered from $\I_2$ to $\I$. 
	%%
	We soon note that $\underD(\I_1)=\underD(\I_2)$, and thus $h_1$ is a mapping from $\underD(\I_2)$ as well. Moreover, since $h_1$ is an homomorphism, then Conditions~1-4 of Definition~\ref{def:homomorphism} are obviously satisfied. It remains to prove that Condition~5 of Definition~\ref{def:homomorphism} is also satisfied, i.e., we have to prove that for each fact  $P(\genericSet_1,\ldots,\genericSet_n)$ in $\I_2$ there exists a fact $P(\genericSettwo_1,\ldots,\genericSettwo_n)$ in $\I$ such that  $h_1(\genericSet_i) \subseteq \genericSettwo_i$, for $1 \leq i \leq n$.
	%%
	We recall that $\I_2$ is obtained by replacing in $\I_1$ every occurrence of $E_1$ and every occurrence of $E_2$ with $E_1 \cup E_2$. Therefore, two cases are possible. $(a)$ $\genericSet_i \neq E_1 \cup E_2$  for $1 \leq i \leq n$. In this case, the thesis holds since $P(\genericSet_1,\ldots,\genericSet_n)$ is also in $\I_1$ and $h_1$ is an homomorphism from $\I_1$ to $\I$. $(b)$ there is $j$ such that $1 \leq j \leq n$ and $\genericSet_j=E_1 \cup E_2$. WLOG we can also assume that $\genericSet_i \neq E_1 \cup E_2$ for $1 \leq i \leq n$ and $i \neq j$. Since two equivalence classes are either disjoint or are the same class, we have that each $T_i$ such that $i\neq j$ is either a set of values or an equivalence class disjoint from $E_1 \cup E_2$.
	%%
	Then, there is a fact $P(\genericSet_1,\ldots,\genericSet_{j-1},\genericSet'_j,\genericSet_{j+1}\ldots,\genericSet_n)$ in $\I_1$ where it is either $\genericSet'_j=E_1$ or $\genericSet'_j=E_2$, and, for every $i\neq j$, $T_i \neq E_1$ and $T_i \neq E_2$ . Let us consider  $\genericSet'_j=E_1$ (the other choice can be treated analogously). Then, there must exist a fact $P(\genericSettwo_1,\ldots,\genericSettwo_{j-1},\genericSettwo_j,\genericSettwo_{j+1}\ldots,\genericSettwo_n)$ in $\I$ such that $h_1(T_i) \subseteq U_i$ for $1 \leq i \leq n$. In particular, this means that $h_1(E_1) \subseteq \genericSettwo_j$, with $\genericSettwo_j$ an equivalence class in $\activeD_E(\I)$. 
	%%
	Since $h_1(E_1) \subseteq E_1'$, it must be $\genericSettwo_j =E_1'$. Indeed, for the two equivalence classes $\genericSettwo_j$  and $E_1'$ it holds either $\genericSettwo_j =E_1'$ or $\genericSettwo_j  \cap E_1'=\emptyset$, but the second option is impossible, since  $h_1(E_1)$ is a common non-empty subset of $\genericSettwo_j$  and $E_1'$. Then, since $\I$ satisfies the entity-egd $d$, which in $d$ is triggered by $\hat{\mu}$, we have that $E_1'=E_2'$ and thus from $h_1(E_1)\subseteq E_1'$ and $h_1(E_2)\subseteq E_2'$ it follows  $h_1(E_1)\cup h_1(E_2)\subseteq E_1'$ and thus $h_1(E_1\cup E_2)\subseteq E_1'$, that is $h_1(\genericSet_j)\subseteq E_1'=U_j$. This shows that $P(\genericSettwo_1,\ldots,\genericSettwo_{j-1},\genericSettwo_j,\genericSettwo_{j+1}\ldots,\genericSettwo_n)$ is the fact in $\I$ we were looking for, thus proving Condition~5 of Definition~\ref{def:homomorphism}.
	
	\emph{Case of value-egd chase step:} The proof is similar to the one used for the entity-egd chase step. 
	%%
	Let $d$ be an entity-egd of the form (\ref{eq:egd}), and, WLOG, assume that $\phi(\vec{x})=P_1(y,z)\land P_2(z)$, where $y,z$ are value-variables (the possible presence of entity-variables, entities and values can be dealt with as shown in the previous cases of this proof). Then, $\tau(\phi(\vec{x}))=P_1(S_1^y,S_1^z)\land P_2(S_2^z)$. Since $\mu$ is assignment from $\phi(\vec{x})$ to $\I_1$, then there exist $V_1,V_2,V_3 \in \activeD_V(\I_1) $ such that $\mu(S_1^y)=V_1$, $\mu(S_1^z)=V_2$, $\mu(S_2^z)=V_3$, $V_2 \cap V_3 \neq \emptyset$, $P_1(V_1,V_2)$ and $P_2(V_3)$ are facts in $\I_1$.
	%%
	Since $h_1$ is homomorphism from $\I_1$ to $\I$, then there are facts in $P_1(V_1',V_2')$ and $P_2(V_3')$ in $\I$ such that $h_1(V_1) \subseteq V_1'$, $h_1(V_2) \subseteq V_2'$, $h_1(V_3) \subseteq V_3'$. Since $V_2 \cap V_3 \neq \emptyset$, then $V_2' \cap V_3' \neq \emptyset$. We define a mapping $\hat{\mu}$ such that $\hat{\mu}(S_1^y)=V_1'$, $\hat{\mu}(S_1^z)=V_2'$, $\hat{\mu}(S_2^z)=V_3'$. It is easy to see that $\hat{\mu}$ is an assignment from $\phi(\vec{x})$ to $\I$.
	
	We then take $h_2$ to be $h_1$ and show that $h_1$ is still a homomorphism when considered from $\I_2$ to $\I$. 
	%%
	We soon note that $\underD(\I_1)=\underD(\I_2)$, and thus $h_1$ is a mapping from $\underD(\I_2)$ as well. Moreover, since $h_1$ is an homomorphism, then condition 1-4 of Definition~\ref{def:homomorphism} are obviously satisfied.
	%%
	Condition~5 of Definition~\ref{def:homomorphism} is also already satisfied for all facts in $\I_2$ that are also in $\I_1$. It remains to prove that such condition holds also for facts in  $\I_2 \setminus \I_1$. The only two such facts are $P_1(V_1 \cup V_2 \cup V_3, V_1 \cup V_2 \cup V_3)$ and $P_2(V_1 \cup V_2 \cup V_3)$ (see the value-egd chase step in Definition~\ref{def:chaseStep}). We have to show that there are facts $P_1(\hat{V_1},\hat{V_2})$ and $P_2(\hat{V_3})$ in $\I$ such that $h_1(V_1 \cup V_2 \cup V_3) \subseteq \hat{V_1}$, $h_1(V_1 \cup V_2 \cup V_3) \subseteq \hat{V_2}$, and $h_1(V_1 \cup V_2 \cup V_3) \subseteq \hat{V_3}$.
	%%
	It is not difficult to see that such facts are $P_1(V_1',V_2')$ and $P_2(V_3')$. Indeed, we know that $h_1(V_1) \subseteq V_1'$ , $h_1(V_2) \subseteq V_2'$ and $h_1(V_3) \subseteq V_3'$. Then, since $\I$ satisfies $d$, which is triggered in $\I$ by $\hat{\mu}$,  it must be $V_1'=V_2'=V_3'$. Thus, we have that $h_1(V_1) \cup h_1(V_2) \cup h_1(V_3) \subseteq V_1'=V_2'=V_3'$, and thus $h_1(V_1 \cup V_2 \cup V_3) \subseteq V_1'=V_2'=V_3'$, which shows the thesis.
\end{proof}


\begin{theorem}
	\label{thm:chase-univ-model}
	Let $\K$ be a KB, and $\sigma=\I_0,\I_1,\ldots,\I_m$ be a finite chase for $\K$. Then $\chase(\K)$ is a universal solution for $\K$. 
\end{theorem}

\begin{proof}
	From Lemma \ref{lem:chase-finite-case-model} it follows that $\chase(\K)$ is a model for $\K$. It remains to prove that it is universal, i.e., that there exists an homomorphism from $\chase(\K)=\I_m$ to every solution for $\K$. The proof is based on Lemma~\ref{lem:triangle-finite-case} and on the observation that the identity mapping $\id$ is a homomorphism from $\I_0$ to every $\I \in \Mod(\K)$. The thesis can be thus proved by applying Lemma~\ref{lem:triangle-finite-case} to each $\I_i,\I_{i+1}$ in $\sigma$, starting from $\I_0,\I_1$, with $h_1=\id$ as homomorphism from $\I_0$ to a solution $\I$ for $\K$. 
\end{proof}

\subsection{Non-terminating chase }

In the presence of an infinite chase sequence, the definition of the result of the chase requires some care. The typical approach adopted in the presence of tgds only~\cite{KrMR19,GoOn19}, or for some settings of \emph{separable} tgds and egds~\cite{JoKl84,CDLLR07,CaGK13}, is to define the result of the chase as t%he structure containing 
the infinite union of all facts %occurring in the structures 
generated in the various chase steps. This approach does not work in the presence of tgds and egds since the resulting %structure 
instance would not satisfy all rules and thus would not be a model (i.e., a solution according to our terminology). Notice also that in our framework the union of all instances in a chase sequence is not even an instance for the KB at hand, because the sets of entities in the result would not correspond to equivalence classes with respect to an equivalence relation (cf.\ Definition~\ref{def:instance}).
Another possibility, which might seem more suited for a setting allowing for general tgds and egds, is to define the result of the chase as the instance %structure 
containing all facts that appear in all instances in the chase sequence from a certain point on, i.e., facts that are introduced in an instance and are never modified in subsequent chase steps. This definition is adopted, e.g., in~\cite{BeVa84}. In our setting, given a KB $\K$ and an infinite chase sequence $\I_0,\I_1,\ldots$, this would mean to define the result of the chase of $\K$, denoted $\chase(\K)$, as follows:
%%
\begin{multline}
\chase(\K)=\{f \mid \textrm{there is some } i\geq 0 \textrm{ such that } \\ f \in \I_j  \textrm{ for each } j \geq i\}.
\end{multline}

The following example shows that this definition is not adequate in our setting, since there are cases in which the above set might be empty (in the presence of a non-empty database $\DB$). 
%(the following example shows that also the infinite union approach does not work, but for this case simpler examples can be devised).

\begin{example}
	\label{exa:phokion}
	Consider the KB $\K=\tup{\T, \DB}$ such that $\T$ is constituted by the following two rules
	
	%\begin{tabular}{ m{6cm}}
	%	{\begin{equation}
			%		E(x,y) \ra E(y,z)
			%			\label{eq:exa-tgd}
			%		\end{equation}}\\[-1.3cm]
	%	{\begin{equation}
			%	E(x,y) \land E(y,z) \ra y=z
			%		\label{eq:exa-egd}
			%\end{equation}}
			%\end{tabular}	
			
			\[
			\begin{array}{ll}
				r_1) & E(x,y) \ra E(y,z)\\
				r_2) &	E(x,y) \land E(y,z) \ra y=z
			\end{array}	
			\]
			where the predicate $E$ is such that $\type(E)=\tup{\val,\val}$,
			and the database $\DB=\{E(1,2)\}$. The chase sequence is constructed starting from $\I_0=\{E(\{1\},\{2\})\}$ 	and by applying indefinitely the above rules in the following order: %%$(\ref{eq:exa-tgd}),(\ref{eq:exa-tgd}),(\ref{eq:exa-egd}),(\ref{eq:exa-tgd}),(\ref{eq:exa-egd}),(\ref{eq:exa-tgd}),\ldots$.
			$r_1,r_1,r_2,r_1,r_2,r_1,r_2,r_1\ldots$.
			
			We obtain a chase sequence $\I_0,\I_1,\ldots$ such that
			\[
			\begin{array}{lcl}
				\I_0&=&\{E(\{1\},\{2\})\}\\
				\I_1&=&\{E(\{1\},\{2\}),E(\{2\},\{v_\bot^1\})\}\\
				\I_2&=&\{E(\{1\},\{2\}),E(\{2\},\{v_\bot^1\}), E(\{v_\bot^1\},\{v_\bot^2\})\}\\
				\I_3&=&\{E(\{1\},\{2,v_\bot^1\}),E(\{2,v_\bot^1\},\{2,v_\bot^1\}), \\
                    && E(\{v_\bot^1\},\{v_\bot^2\})\}\\
				\I_4&=&\{E(\{1\},\{2,v_\bot^1\}),E(\{2,v_\bot^1\},\{2,v_\bot^1\}), \\
                    && E(\{v_\bot^1\},\{v_\bot^2\}),E(\{v_\bot^2\},\{v_\bot^3\})\}\\
				\I_5&=&\{E(\{1\},\{2,v_\bot^1,v_\bot^2\}),E(\{2,v_\bot^1\},\{2,v_\bot^1\}), \\
                    && E(\{2,v_\bot^1,v_\bot^2\},\{2,v_\bot^1,v_\bot^2\}),E(\{v_\bot^2\},\{v_\bot^3\})\}\\
				\I_6&=&\{E(\{1\},\{2,v_\bot^1,v_\bot^2\}),E(\{2,v_\bot^1\},\{2,v_\bot^1\}), \\
                    && E(\{2,v_\bot^1,v_\bot^2\},\{2,v_\bot^1,v_\bot^2\}),E(\{v_\bot^2\},\{v_\bot^3\}), \\ 
                    && E(\{v_\bot^3\},\{v_\bot^4\})\}\\
				\I_7&=&\{E(\{1\},\{2,v_\bot^1,v_\bot^2\}),E(\{2,v_\bot^1\},\{2,v_\bot^1,v_\bot^2\}), \\ 
                    && E(\{2,v_\bot^1,v_\bot^2\},\{2,v_\bot^1,v_\bot^2\}),E(\{v_\bot^2\},\{v_\bot^3\}),\\ 
                    && E(\{v_\bot^3\},\{v_\bot^4\})\}\\
				\ldots
			\end{array}
			\]
			
			We point out that in the step $\I_2 \xrightarrow[]{r_2,\mu_2} \I_3$, the image of $\mu_2$ is given by the facts $\{E(\{1\},\{2\}),E(\{2\},\{v_\bot^1\})$; in the step $\I_4 \xrightarrow[]{r_2,\mu_4} \I_5$, the image of $\mu_4$ is given by the facts $\{E(\{1\},\{2,v_\bot^1\}),E(\{v_\bot^1\},\{v_\bot^2\})$; in the step $\I_6 \xrightarrow[]{r_2,\mu_6} \I_7$, the image of $\mu_6$ is given by the facts $E(\{2,v_\bot^1\},\{2,v_\bot^1\}),E(\{2,v_\bot^1,v_\bot^2\},\{2,v_\bot^1,v_\bot^2\})$.
			
			It is not difficult to see that, given the above infinite sequence $\I_0,\I_1,\ldots$,
			%no fact occur from a certain point on or not even infinitely often
			the set $\chase(\K)$ as defined above is empty.\nb{notice that all triggers existing in $\I_3$ have been executed, that is the chase sequence we are constructing can be considered fair. Notice also that if we would execute all egds before the tgds, we would obtain a finite chase (however, we need to ensure to have a result of the chase for any arbitrary order)
			}	
			\qed
		\end{example}
		

